Poles of degenerate Eisenstein series and Siegel-Weil identities for exceptional split groups

Let $G$ be a linear split algebraic group. The degenerate Eisenstein series associated to a maximal parabolic subgroup $E_{P}(f^{0},s,g)$ with the spherical section $f^{0}$ is studied in the first part of the thesis. In this part, we study the poles of $E_{P}(f^{0},s,g)$ in the region $\operatorname{Re} s >0$. We determine when the leading term in the Laurent expansion of $E_{P}(f^{0},s,g)$ around $s=s_0$ is square integrable. The second part is devoted to finding identities between the leading terms of various Eisenstein series at different points. We present an algorithm to find this data and implement it on \textit{SAGE}. While both parts can be applied to a general algebraic group, we restrict ourself to the case where $G$ is split exceptional group of type $F_4,E_6,E_7$, and obtain new results.

==> Appendices/ids/E6.tex <==
\begin{landscape} 
  \begin{table} 
 \caption{$E_{6}$ Parabolic 1 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{12} $ & $ \left[1, 1, 12 s, -12 s + 1, 12 s, -12 s + 1\right] $ & $ w_{6}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{1}{12} \le s < \frac{1}{6} $ & $ \left[1, -12 s + 2, 1, 12 s - 1, -12 s + 2, 12 s - 1\right] $ & $ w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{1}{6} \le s < \frac{1}{4} $ & $ \left[1, 12 s - 2, 1, -12 s + 3, 12 s - 2, 1\right] $ & $ w_{4}w_{3}w_{1} $ \\
$ \frac{1}{4} \le s < \frac{1}{3} $ & $ \left[1, 1, -12 s + 4, 12 s - 3, 1, 1\right] $ & $ w_{3}w_{1} $ \\
$ \frac{1}{3} \le s < \frac{5}{12} $ & $ \left[-12 s + 5, 1, 12 s - 4, 1, 1, 1\right] $ & $ w_{1} $ \\
$ \frac{5}{12} \le s \le \frac{1}{2} $ & $ \left[12 s - 5, 1, 1, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 6 }$ Parabolic 2 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{22} $ & $ \left[1, -11 s + \frac{1}{2}, -11 s + \frac{1}{2}, 22 s, -11 s + \frac{1}{2}, 1\right] $ & $ w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{1}{22} \le s < \frac{3}{22} $ & $ \left[-11 s + \frac{3}{2}, 11 s - \frac{1}{2}, 11 s - \frac{1}{2}, -11 s + \frac{3}{2}, 11 s - \frac{1}{2}, -11 s + \frac{3}{2}\right] $ & $ w_{6}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{3}{22} \le s < \frac{5}{22} $ & $ \left[11 s - \frac{3}{2}, 1, -11 s + \frac{5}{2}, 11 s - \frac{3}{2}, -11 s + \frac{5}{2}, 11 s - \frac{3}{2}\right] $ & $ w_{5}w_{3}w_{4}w_{2} $ \\
$ \frac{5}{22} \le s < \frac{7}{22} $ & $ \left[1, 1, 11 s - \frac{5}{2}, -11 s + \frac{7}{2}, 11 s - \frac{5}{2}, 1\right] $ & $ w_{4}w_{2} $ \\
$ \frac{7}{22} \le s < \frac{9}{22} $ & $ \left[1, -11 s + \frac{9}{2}, 1, 11 s - \frac{7}{2}, 1, 1\right] $ & $ w_{2} $ \\
$ \frac{9}{22} \le s \le \frac{1}{2} $ & $ \left[1, 11 s - \frac{9}{2}, 1, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 6 }$ Parabolic 3 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{18} $ & $ \left[9 s + \frac{1}{2}, -9 s + \frac{1}{2}, -9 s + \frac{1}{2}, 18 s, -9 s + \frac{1}{2}, -9 s + \frac{1}{2}\right] $ & $ w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{18} \le s < \frac{1}{9} $ & $ \left[1, 9 s - \frac{1}{2}, 9 s - \frac{1}{2}, -18 s + 2, 9 s - \frac{1}{2}, 9 s - \frac{1}{2}\right] $ & $ w_{4}w_{5}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{9} \le s < \frac{1}{6} $ & $ \left[1, -9 s + \frac{3}{2}, -9 s + \frac{3}{2}, 18 s - 2, -9 s + \frac{3}{2}, 9 s - \frac{1}{2}\right] $ & $ w_{5}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{6} \le s < \frac{5}{18} $ & $ \left[-9 s + \frac{5}{2}, 9 s - \frac{3}{2}, 9 s - \frac{3}{2}, -9 s + \frac{5}{2}, 9 s - \frac{3}{2}, 1\right] $ & $ w_{4}w_{1}w_{3} $ \\
$ \frac{5}{18} \le s < \frac{7}{18} $ & $ \left[9 s - \frac{5}{2}, 1, -9 s + \frac{7}{2}, 9 s - \frac{5}{2}, 1, 1\right] $ & $ w_{3} $ \\
$ \frac{7}{18} \le s \le \frac{1}{2} $ & $ \left[1, 1, 9 s - \frac{7}{2}, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 6 }$ Parabolic 4 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{42} $ & $ \left[-7 s + \frac{1}{2}, 14 s, 14 s, -21 s + \frac{1}{2}, 14 s, -7 s + \frac{1}{2}\right] $ & $ w_{4}w_{5}w_{6}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{42} \le s < \frac{1}{14} $ & $ \left[-7 s + \frac{1}{2}, -7 s + \frac{1}{2}, -7 s + \frac{1}{2}, 21 s - \frac{1}{2}, -7 s + \frac{1}{2}, -7 s + \frac{1}{2}\right] $ & $ w_{5}w_{6}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{14} \le s < \frac{1}{7} $ & $ \left[7 s - \frac{1}{2}, 7 s - \frac{1}{2}, 7 s - \frac{1}{2}, -14 s + 2, 7 s - \frac{1}{2}, 7 s - \frac{1}{2}\right] $ & $ w_{4}w_{5}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{7} \le s < \frac{3}{14} $ & $ \left[7 s - \frac{1}{2}, -7 s + \frac{3}{2}, -7 s + \frac{3}{2}, 14 s - 2, -7 s + \frac{3}{2}, 7 s - \frac{1}{2}\right] $ & $ w_{5}w_{3}w_{2}w_{4} $ \\
$ \frac{3}{14} \le s < \frac{5}{14} $ & $ \left[1, 7 s - \frac{3}{2}, 7 s - \frac{3}{2}, -7 s + \frac{5}{2}, 7 s - \frac{3}{2}, 1\right] $ & $ w_{4} $ \\
$ \frac{5}{14} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 7 s - \frac{5}{2}, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 6 }$ Parabolic 5 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{18} $ & $ \left[-9 s + \frac{1}{2}, -9 s + \frac{1}{2}, -9 s + \frac{1}{2}, 18 s, -9 s + \frac{1}{2}, 9 s + \frac{1}{2}\right] $ & $ w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{18} \le s < \frac{1}{9} $ & $ \left[9 s - \frac{1}{2}, 9 s - \frac{1}{2}, 9 s - \frac{1}{2}, -18 s + 2, 9 s - \frac{1}{2}, 1\right] $ & $ w_{4}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{9} \le s < \frac{1}{6} $ & $ \left[9 s - \frac{1}{2}, -9 s + \frac{3}{2}, -9 s + \frac{3}{2}, 18 s - 2, -9 s + \frac{3}{2}, 1\right] $ & $ w_{5}w_{6}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{6} \le s < \frac{5}{18} $ & $ \left[1, 9 s - \frac{3}{2}, 9 s - \frac{3}{2}, -9 s + \frac{5}{2}, 9 s - \frac{3}{2}, -9 s + \frac{5}{2}\right] $ & $ w_{6}w_{4}w_{5} $ \\
$ \frac{5}{18} \le s < \frac{7}{18} $ & $ \left[1, 1, 1, 9 s - \frac{5}{2}, -9 s + \frac{7}{2}, 9 s - \frac{5}{2}\right] $ & $ w_{5} $ \\
$ \frac{7}{18} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 1, 9 s - \frac{7}{2}, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 6 }$ Parabolic 6 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{12} $ & $ \left[-12 s + 1, 1, 12 s, -12 s + 1, 12 s, 1\right] $ & $ w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{1}{12} \le s < \frac{1}{6} $ & $ \left[12 s - 1, -12 s + 2, -12 s + 2, 12 s - 1, 1, 1\right] $ & $ w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{1}{6} \le s < \frac{1}{4} $ & $ \left[1, 12 s - 2, 12 s - 2, -12 s + 3, 1, 1\right] $ & $ w_{4}w_{5}w_{6} $ \\
$ \frac{1}{4} \le s < \frac{1}{3} $ & $ \left[1, 1, 1, 12 s - 3, -12 s + 4, 1\right] $ & $ w_{5}w_{6} $ \\
$ \frac{1}{3} \le s < \frac{5}{12} $ & $ \left[1, 1, 1, 1, 12 s - 4, -12 s + 5\right] $ & $ w_{6} $ \\
$ \frac{5}{12} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 1, 1, 12 s - 5\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape}

==> Appendices/ids/E7.tex <==
\begin{landscape} 
  \begin{table} 
 \caption{$E_{7}$ Parabolic 1 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{34} $ & $ \left[1, -17 s + \frac{1}{2}, -17 s + \frac{1}{2}, 34 s, -17 s + \frac{1}{2}, 1, 1\right] $ & $ w_{5}w_{6}w_{7}w_{3}w_{2}w_{4}w_{5}w_{6}w_{1}w_{3}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{1}{34} \le s < \frac{3}{34} $ & $ \left[-17 s + \frac{3}{2}, 17 s - \frac{1}{2}, 17 s - \frac{1}{2}, -17 s + \frac{3}{2}, 17 s - \frac{1}{2}, -17 s + \frac{3}{2}, 1\right] $ & $ w_{6}w_{7}w_{4}w_{5}w_{6}w_{1}w_{3}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{3}{34} \le s < \frac{5}{34} $ & $ \left[17 s - \frac{3}{2}, 1, -17 s + \frac{5}{2}, 17 s - \frac{3}{2}, -17 s + \frac{5}{2}, 17 s - \frac{3}{2}, -17 s + \frac{5}{2}\right] $ & $ w_{7}w_{5}w_{6}w_{3}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{5}{34} \le s < \frac{7}{34} $ & $ \left[1, 1, 17 s - \frac{5}{2}, -17 s + \frac{7}{2}, 17 s - \frac{5}{2}, -17 s + \frac{7}{2}, 17 s - \frac{5}{2}\right] $ & $ w_{6}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{7}{34} \le s < \frac{9}{34} $ & $ \left[1, -17 s + \frac{9}{2}, 1, 17 s - \frac{7}{2}, -17 s + \frac{9}{2}, 17 s - \frac{7}{2}, 1\right] $ & $ w_{5}w_{2}w_{4}w_{3}w_{1} $ \\
$ \frac{9}{34} \le s < \frac{11}{34} $ & $ \left[1, 17 s - \frac{9}{2}, 1, -17 s + \frac{11}{2}, 17 s - \frac{9}{2}, 1, 1\right] $ & $ w_{4}w_{3}w_{1} $ \\
$ \frac{11}{34} \le s < \frac{13}{34} $ & $ \left[1, 1, -17 s + \frac{13}{2}, 17 s - \frac{11}{2}, 1, 1, 1\right] $ & $ w_{3}w_{1} $ \\
$ \frac{13}{34} \le s < \frac{15}{34} $ & $ \left[-17 s + \frac{15}{2}, 1, 17 s - \frac{13}{2}, 1, 1, 1, 1\right] $ & $ w_{1} $ \\
$ \frac{15}{34} \le s \le \frac{1}{2} $ & $ \left[17 s - \frac{15}{2}, 1, 1, 1, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 2 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{28} $ & $ \left[14 s, 14 s, 14 s, -28 s + 1, 14 s, -14 s + 1, 14 s\right] $ & $ w_{4}w_{5}w_{6}w_{7}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{3}w_{2}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{1}{28} \le s < \frac{1}{14} $ & $ \left[14 s, -14 s + 1, -14 s + 1, 28 s - 1, -14 s + 1, -14 s + 1, 14 s\right] $ & $ w_{5}w_{6}w_{7}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{3}w_{2}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{1}{14} \le s < \frac{3}{28} $ & $ \left[1, 14 s - 1, 14 s - 1, -28 s + 3, 14 s - 1, 14 s - 1, -14 s + 2\right] $ & $ w_{7}w_{4}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{3}{28} \le s < \frac{1}{7} $ & $ \left[1, -14 s + 2, -14 s + 2, 28 s - 3, -14 s + 2, 14 s - 1, -14 s + 2\right] $ & $ w_{7}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{1}{7} \le s < \frac{3}{14} $ & $ \left[-14 s + 3, 14 s - 2, 14 s - 2, -14 s + 3, 14 s - 2, -14 s + 3, 14 s - 2\right] $ & $ w_{6}w_{4}w_{5}w_{1}w_{3}w_{4}w_{2} $ \\
$ \frac{3}{14} \le s < \frac{2}{7} $ & $ \left[14 s - 3, 1, -14 s + 4, 14 s - 3, -14 s + 4, 14 s - 3, 1\right] $ & $ w_{5}w_{3}w_{4}w_{2} $ \\
$ \frac{2}{7} \le s < \frac{5}{14} $ & $ \left[1, 1, 14 s - 4, -14 s + 5, 14 s - 4, 1, 1\right] $ & $ w_{4}w_{2} $ \\
$ \frac{5}{14} \le s < \frac{3}{7} $ & $ \left[1, -14 s + 6, 1, 14 s - 5, 1, 1, 1\right] $ & $ w_{2} $ \\
$ \frac{3}{7} \le s \le \frac{1}{2} $ & $ \left[1, 14 s - 6, 1, 1, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 3 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{66} $ & $ \left[-11 s + \frac{1}{2}, 22 s, 22 s, -33 s + \frac{1}{2}, 22 s, -11 s + \frac{1}{2}, 1\right] $ & $ w_{4}w_{5}w_{6}w_{7}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{66} \le s < \frac{1}{22} $ & $ \left[-11 s + \frac{1}{2}, -11 s + \frac{1}{2}, -11 s + \frac{1}{2}, 33 s - \frac{1}{2}, -11 s + \frac{1}{2}, -11 s + \frac{1}{2}, 1\right] $ & $ w_{5}w_{6}w_{7}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{22} \le s < \frac{1}{11} $ & $ \left[11 s - \frac{1}{2}, 11 s - \frac{1}{2}, 11 s - \frac{1}{2}, -22 s + 2, 11 s - \frac{1}{2}, 11 s - \frac{1}{2}, -22 s + 2\right] $ & $ w_{7}w_{4}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{1}{11} \le s < \frac{3}{22} $ & $ \left[11 s - \frac{1}{2}, -11 s + \frac{3}{2}, -11 s + \frac{3}{2}, 22 s - 2, -11 s + \frac{3}{2}, -11 s + \frac{3}{2}, 22 s - 2\right] $ & $ w_{5}w_{6}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{3}{22} \le s < \frac{2}{11} $ & $ \left[1, 11 s - \frac{3}{2}, 11 s - \frac{3}{2}, -22 s + 4, 11 s - \frac{3}{2}, 11 s - \frac{3}{2}, 1\right] $ & $ w_{4}w_{5}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{2}{11} \le s < \frac{5}{22} $ & $ \left[1, -11 s + \frac{5}{2}, -11 s + \frac{5}{2}, 22 s - 4, -11 s + \frac{5}{2}, 11 s - \frac{3}{2}, 1\right] $ & $ w_{5}w_{3}w_{2}w_{4}w_{1}w_{3} $ \\
$ \frac{5}{22} \le s < \frac{7}{22} $ & $ \left[-11 s + \frac{7}{2}, 11 s - \frac{5}{2}, 11 s - \frac{5}{2}, -11 s + \frac{7}{2}, 11 s - \frac{5}{2}, 1, 1\right] $ & $ w_{4}w_{1}w_{3} $ \\
$ \frac{7}{22} \le s < \frac{9}{22} $ & $ \left[11 s - \frac{7}{2}, 1, -11 s + \frac{9}{2}, 11 s - \frac{7}{2}, 1, 1, 1\right] $ & $ w_{3} $ \\
$ \frac{9}{22} \le s \le \frac{1}{2} $ & $ \left[1, 1, 11 s - \frac{9}{2}, 1, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 4 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{32} $ & $ \left[8 s, 8 s, 8 s, 8 s, -32 s + 1, 8 s, 8 s\right] $ & $ w_{5}w_{6}w_{7}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{32} \le s < \frac{1}{24} $ & $ \left[8 s, 8 s, 8 s, -24 s + 1, 32 s - 1, -24 s + 1, 8 s\right] $ & $ w_{6}w_{7}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{24} \le s < \frac{1}{16} $ & $ \left[8 s, -16 s + 1, -16 s + 1, 24 s - 1, -16 s + 1, 24 s - 1, -16 s + 1\right] $ & $ w_{7}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{16} \le s < \frac{1}{12} $ & $ \left[-8 s + 1, 16 s - 1, 16 s - 1, -24 s + 2, 16 s - 1, -8 s + 1, 16 s - 1\right] $ & $ w_{4}w_{5}w_{6}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{12} \le s < \frac{1}{8} $ & $ \left[-8 s + 1, -8 s + 1, -8 s + 1, 24 s - 2, -8 s + 1, -8 s + 1, 16 s - 1\right] $ & $ w_{5}w_{6}w_{1}w_{3}w_{2}w_{4}w_{5}w_{4}w_{1}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{8} \le s < \frac{3}{16} $ & $ \left[8 s - 1, 8 s - 1, 8 s - 1, -16 s + 3, 8 s - 1, 8 s - 1, 1\right] $ & $ w_{4}w_{5}w_{3}w_{2}w_{4} $ \\
$ \frac{3}{16} \le s < \frac{1}{4} $ & $ \left[8 s - 1, -8 s + 2, -8 s + 2, 16 s - 3, -8 s + 2, 8 s - 1, 1\right] $ & $ w_{5}w_{3}w_{2}w_{4} $ \\
$ \frac{1}{4} \le s < \frac{3}{8} $ & $ \left[1, 8 s - 2, 8 s - 2, -8 s + 3, 8 s - 2, 1, 1\right] $ & $ w_{4} $ \\
$ \frac{3}{8} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 8 s - 3, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 5 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{30} $ & $ \left[10 s, 10 s, 10 s, -30 s + 1, 10 s, 10 s, 10 s\right] $ & $ w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{30} \le s < \frac{1}{20} $ & $ \left[10 s, -20 s + 1, -20 s + 1, 30 s - 1, -20 s + 1, 10 s, 10 s\right] $ & $ w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{20} \le s < \frac{1}{15} $ & $ \left[-10 s + 1, 20 s - 1, 20 s - 1, -30 s + 2, 20 s - 1, -10 s + 1, 10 s\right] $ & $ w_{4}w_{5}w_{6}w_{7}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{15} \le s < \frac{1}{10} $ & $ \left[-10 s + 1, -10 s + 1, -10 s + 1, 30 s - 2, -10 s + 1, -10 s + 1, 10 s\right] $ & $ w_{5}w_{6}w_{7}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{10} \le s < \frac{3}{20} $ & $ \left[10 s - 1, 10 s - 1, 10 s - 1, -20 s + 3, 10 s - 1, 10 s - 1, -10 s + 2\right] $ & $ w_{7}w_{4}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{3}{20} \le s < \frac{1}{5} $ & $ \left[10 s - 1, -10 s + 2, -10 s + 2, 20 s - 3, -10 s + 2, 10 s - 1, -10 s + 2\right] $ & $ w_{7}w_{5}w_{6}w_{3}w_{2}w_{4}w_{5} $ \\
$ \frac{1}{5} \le s < \frac{3}{10} $ & $ \left[1, 10 s - 2, 10 s - 2, -10 s + 3, 10 s - 2, -10 s + 3, 10 s - 2\right] $ & $ w_{6}w_{4}w_{5} $ \\
$ \frac{3}{10} \le s < \frac{2}{5} $ & $ \left[1, 1, 1, 10 s - 3, -10 s + 4, 10 s - 3, 1\right] $ & $ w_{5} $ \\
$ \frac{2}{5} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 1, 10 s - 4, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 6 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{26} $ & $ \left[1, -13 s + \frac{1}{2}, -13 s + \frac{1}{2}, 26 s, -13 s + \frac{1}{2}, -13 s + \frac{1}{2}, 26 s\right] $ & $ w_{6}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{1}{26} \le s < \frac{1}{13} $ & $ \left[-13 s + \frac{3}{2}, 13 s - \frac{1}{2}, 13 s - \frac{1}{2}, -26 s + 2, 13 s - \frac{1}{2}, 13 s - \frac{1}{2}, 1\right] $ & $ w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{1}{13} \le s < \frac{3}{26} $ & $ \left[-13 s + \frac{3}{2}, -13 s + \frac{3}{2}, -13 s + \frac{3}{2}, 26 s - 2, -13 s + \frac{3}{2}, 13 s - \frac{1}{2}, 1\right] $ & $ w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{3}{26} \le s < \frac{2}{13} $ & $ \left[13 s - \frac{3}{2}, 13 s - \frac{3}{2}, 13 s - \frac{3}{2}, -26 s + 4, 13 s - \frac{3}{2}, 1, 1\right] $ & $ w_{4}w_{5}w_{6}w_{7}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{2}{13} \le s < \frac{5}{26} $ & $ \left[13 s - \frac{3}{2}, -13 s + \frac{5}{2}, -13 s + \frac{5}{2}, 26 s - 4, -13 s + \frac{5}{2}, 1, 1\right] $ & $ w_{5}w_{6}w_{7}w_{3}w_{2}w_{4}w_{5}w_{6} $ \\
$ \frac{5}{26} \le s < \frac{7}{26} $ & $ \left[1, 13 s - \frac{5}{2}, 13 s - \frac{5}{2}, -13 s + \frac{7}{2}, 13 s - \frac{5}{2}, -13 s + \frac{7}{2}, 1\right] $ & $ w_{6}w_{7}w_{4}w_{5}w_{6} $ \\
$ \frac{7}{26} \le s < \frac{9}{26} $ & $ \left[1, 1, 1, 13 s - \frac{7}{2}, -13 s + \frac{9}{2}, 13 s - \frac{7}{2}, -13 s + \frac{9}{2}\right] $ & $ w_{7}w_{5}w_{6} $ \\
$ \frac{9}{26} \le s < \frac{11}{26} $ & $ \left[1, 1, 1, 1, 13 s - \frac{9}{2}, -13 s + \frac{11}{2}, 13 s - \frac{9}{2}\right] $ & $ w_{6} $ \\
$ \frac{11}{26} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 1, 1, 13 s - \frac{11}{2}, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ E _{ 7 }$ Parabolic 7 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{18} $ & $ \left[1, 18 s, 1, -18 s + 1, 18 s, -18 s + 1, 18 s\right] $ & $ w_{6}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7} $ \\
$ \frac{1}{18} \le s < \frac{1}{9} $ & $ \left[1, 1, -18 s + 2, 18 s - 1, -18 s + 2, 18 s - 1, 1\right] $ & $ w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7} $ \\
$ \frac{1}{9} \le s < \frac{1}{6} $ & $ \left[-18 s + 3, 1, 18 s - 2, -18 s + 3, 18 s - 2, 1, 1\right] $ & $ w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7} $ \\
$ \frac{1}{6} \le s < \frac{2}{9} $ & $ \left[18 s - 3, -18 s + 4, -18 s + 4, 18 s - 3, 1, 1, 1\right] $ & $ w_{3}w_{2}w_{4}w_{5}w_{6}w_{7} $ \\
$ \frac{2}{9} \le s < \frac{5}{18} $ & $ \left[1, 18 s - 4, 18 s - 4, -18 s + 5, 1, 1, 1\right] $ & $ w_{4}w_{5}w_{6}w_{7} $ \\
$ \frac{5}{18} \le s < \frac{1}{3} $ & $ \left[1, 1, 1, 18 s - 5, -18 s + 6, 1, 1\right] $ & $ w_{5}w_{6}w_{7} $ \\
$ \frac{1}{3} \le s < \frac{7}{18} $ & $ \left[1, 1, 1, 1, 18 s - 6, -18 s + 7, 1\right] $ & $ w_{6}w_{7} $ \\
$ \frac{7}{18} \le s < \frac{4}{9} $ & $ \left[1, 1, 1, 1, 1, 18 s - 7, -18 s + 8\right] $ & $ w_{7} $ \\
$ \frac{4}{9} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 1, 1, 1, 18 s - 8\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape}

==> Appendices/ids/F4.tex <==
\begin{landscape} 
  \begin{table} 
 \caption{$F_{4}$ Parabolic 1 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{16} $ & $ \left[8 s, 8 s, -16 s + 1, 1\right] $ & $ w_{3}w_{4}w_{2}w_{3}w_{2}w_{1} $ \\
$ \frac{1}{16} \le s < \frac{1}{8} $ & $ \left[8 s, -8 s + 1, 16 s - 1, -16 s + 2\right] $ & $ w_{4}w_{2}w_{3}w_{2}w_{1} $ \\
$ \frac{1}{8} \le s < \frac{3}{16} $ & $ \left[1, 8 s - 1, -16 s + 3, 16 s - 2\right] $ & $ w_{3}w_{2}w_{1} $ \\
$ \frac{3}{16} \le s < \frac{1}{4} $ & $ \left[1, -8 s + 2, 16 s - 3, 1\right] $ & $ w_{2}w_{1} $ \\
$ \frac{1}{4} \le s < \frac{3}{8} $ & $ \left[-8 s + 3, 8 s - 2, 1, 1\right] $ & $ w_{1} $ \\
$ \frac{3}{8} \le s \le \frac{1}{2} $ & $ \left[8 s - 3, 1, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ F _{ 4 }$ Parabolic 2 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{30} $ & $ \left[10 s, -15 s + \frac{1}{2}, 10 s, 10 s\right] $ & $ w_{2}w_{3}w_{4}w_{1}w_{2}w_{3}w_{1}w_{2} $ \\
$ \frac{1}{30} \le s < \frac{1}{20} $ & $ \left[-5 s + \frac{1}{2}, 15 s - \frac{1}{2}, -20 s + 1, 10 s\right] $ & $ w_{3}w_{4}w_{1}w_{2}w_{3}w_{1}w_{2} $ \\
$ \frac{1}{20} \le s < \frac{1}{10} $ & $ \left[-5 s + \frac{1}{2}, -5 s + \frac{1}{2}, 20 s - 1, -10 s + 1\right] $ & $ w_{4}w_{1}w_{2}w_{3}w_{1}w_{2} $ \\
$ \frac{1}{10} \le s < \frac{1}{5} $ & $ \left[5 s - \frac{1}{2}, 5 s - \frac{1}{2}, -10 s + 2, 10 s - 1\right] $ & $ w_{3}w_{2} $ \\
$ \frac{1}{5} \le s < \frac{3}{10} $ & $ \left[5 s - \frac{1}{2}, -5 s + \frac{3}{2}, 10 s - 2, 1\right] $ & $ w_{2} $ \\
$ \frac{3}{10} \le s \le \frac{1}{2} $ & $ \left[1, 5 s - \frac{3}{2}, 1, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ F _{ 4 }$ Parabolic 3 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{42} $ & $ \left[-7 s + \frac{1}{2}, 14 s, -21 s + \frac{1}{2}, 14 s\right] $ & $ w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ \\
$ \frac{1}{42} \le s < \frac{1}{14} $ & $ \left[-7 s + \frac{1}{2}, -7 s + \frac{1}{2}, 21 s - \frac{1}{2}, -7 s + \frac{1}{2}\right] $ & $ w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ \\
$ \frac{1}{14} \le s < \frac{1}{7} $ & $ \left[7 s - \frac{1}{2}, 7 s - \frac{1}{2}, -14 s + 2, 7 s - \frac{1}{2}\right] $ & $ w_{3}w_{4}w_{2}w_{3} $ \\
$ \frac{1}{7} \le s < \frac{3}{14} $ & $ \left[7 s - \frac{1}{2}, -7 s + \frac{3}{2}, 14 s - 2, -7 s + \frac{3}{2}\right] $ & $ w_{4}w_{2}w_{3} $ \\
$ \frac{3}{14} \le s < \frac{5}{14} $ & $ \left[1, 7 s - \frac{3}{2}, -7 s + \frac{5}{2}, 7 s - \frac{3}{2}\right] $ & $ w_{3} $ \\
$ \frac{5}{14} \le s \le \frac{1}{2} $ & $ \left[1, 1, 7 s - \frac{5}{2}, 1\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape} \begin{landscape} 
  \begin{table} 
 \caption{$ F _{ 4 }$ Parabolic 4 dom weight} 
 \begin{tabular}{ccc}
Range & dom weight  & w \\
$ 0 \le s < \frac{1}{22} $ & $ \left[1, -11 s + \frac{1}{2}, 22 s, -11 s + \frac{1}{2}\right] $ & $ w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4} $ \\
$ \frac{1}{22} \le s < \frac{3}{22} $ & $ \left[-11 s + \frac{3}{2}, 11 s - \frac{1}{2}, -11 s + \frac{3}{2}, 11 s - \frac{1}{2}\right] $ & $ w_{3}w_{1}w_{2}w_{3}w_{4} $ \\
$ \frac{3}{22} \le s < \frac{5}{22} $ & $ \left[11 s - \frac{3}{2}, -11 s + \frac{5}{2}, 11 s - \frac{3}{2}, 1\right] $ & $ w_{2}w_{3}w_{4} $ \\
$ \frac{5}{22} \le s < \frac{7}{22} $ & $ \left[1, 11 s - \frac{5}{2}, -11 s + \frac{7}{2}, 1\right] $ & $ w_{3}w_{4} $ \\
$ \frac{7}{22} \le s < \frac{9}{22} $ & $ \left[1, 1, 11 s - \frac{7}{2}, -11 s + \frac{9}{2}\right] $ & $ w_{4} $ \\
$ \frac{9}{22} \le s \le \frac{1}{2} $ & $ \left[1, 1, 1, 11 s - \frac{9}{2}\right] $ & $ 1 $ \\
\end{tabular} \end{table} 
  \end{landscape}

==> Chapters/E8.tex <==
\newpage
\lhead{Chapter \ref{ch3:ids}. \emph{Identities- Group of type $E_{8}$}}
\section{Group of type $E_{8}$}
\begin{prop}\label{E8_mod_char} 
The matrix $B$ for $G=E_8$ is
 $$B= \left(\begin{array}{rrrrrrrr}
23 & 8 & 2 & 3 & 5 & 8 & 12 & 17 \\
12 & 17 & 7 & 2 & 5 & 8 & 11 & 14 \\
12 & 8 & 13 & 3 & 5 & 7 & 9 & 11 \\
8 & 8 & 7 & 9 & 5 & 6 & 7 & 8 \\
9 & 8 & 7 & 5 & 11 & 8 & 9 & 10 \\
10 & 8 & 7 & 5 & 4 & 14 & 12 & 13 \\
11 & 8 & 7 & 5 & 4 & 3 & 19 & 18 \\
12 & 8 & 7 & 5 & 4 & 3 & 2 & 29
\end{array}\right) $$ 
 \end{prop} \ 
 \begin{prop} 
 The suitable pairs are as follows: 
 \begin{figure}[H] \begin{center} \begin{tabular}{|c|c|c|c|Hc|c|c|c|} \hline
[s,t] & $\para{P}_{1}$ & $\para{P}_{2}$ & $\para{P}_{3}$ & $\para{P}_{4}$ & $\para{P}_{5}$ & $\para{P}_{6}$ & $\para{P}_{7}$ & $\para{P}_{8}$ \\ %\hline
$\para{P}_{1}$ &  &  &  &  &  &  &  & $\left[\frac{11}{46}, \frac{5}{58}\right]$ \\ %\hline
$\para{P}_{2}$ & $\left[\frac{7}{34}, \frac{7}{46}\right]$ &  &  &  &  &  & $\left[\frac{5}{34}, \frac{3}{38}\right]$ & $\left[\frac{11}{34}, \frac{13}{58}\right]$ \\ %\hline
$\para{P}_{3}$ & $\left[\frac{11}{26}, \frac{19}{46}\right]$ & $\left[\frac{3}{26}, \frac{3}{34}\right]$ &  &  &  & $\left[\frac{1}{26}, 0\right]$ & $\left[\frac{5}{26}, \frac{5}{38}\right]$ & $\left[\frac{9}{26}, \frac{15}{58}\right]$ \\ %\hline
$\para{P}_{4}$ & $\left[\frac{7}{18}, \frac{17}{46}\right]$ & $\left[\frac{7}{18}, \frac{13}{34}\right]$ & $\left[\frac{5}{18}, \frac{7}{26}\right]$ &  & $\left[\frac{1}{18}, \frac{1}{22}\right]$ & $\left[\frac{1}{6}, \frac{1}{7}\right]$ & $\left[\frac{5}{18}, \frac{9}{38}\right]$ & $\left[\frac{7}{18}, \frac{19}{58}\right]$ \\
% \hline
$\para{P}_{5}$ & $\left[\frac{7}{22}, \frac{13}{46}\right]$ & $\left[\frac{5}{22}, \frac{7}{34}\right]$ & $\left[\frac{3}{22}, \frac{3}{26}\right]$ &  &  & $\left[\frac{5}{22}, \frac{3}{14}\right]$ & $\left[\frac{7}{22}, \frac{11}{38}\right]$ & $\left[\frac{9}{22}, \frac{21}{58}\right]$ \\ %\hline
$\para{P}_{6}$ & $\left[\frac{3}{14}, \frac{7}{46}\right]$ & $\left[\frac{1}{14}, \frac{1}{34}\right]$ &  &  &  &  & $\left[\frac{5}{14}, \frac{13}{38}\right]$ & $\left[\frac{3}{7}, \frac{23}{58}\right]$ \\ %\hline
$\para{P}_{7}$ &  &  &  &  &  &  &  & $\left[\frac{17}{38}, \frac{25}{58}\right]$ \\ \hline
%$\para{P}_{8}$ &  &  &  &  &  &  &  &  \\ \hline
\end{tabular} \end{center} 
 \end{figure} 
 \end{prop} \begin{prop} It holds that : 
 \begin{align*} 
 A_{w_{\para{P}_{1} }} = &\frac{R^{7}}{\zeta ( 2 ) \zeta ( 4 ) \zeta ( 6 ) \zeta ( 7 ) \zeta ( 8 ) \zeta ( 10 ) \zeta ( 12 )} \\
 A_{w_{\para{P}_{2} }} = &\frac{R^{7}}{\zeta ( 2 ) \zeta ( 3 ) \zeta ( 4 ) \zeta ( 5 ) \zeta ( 6 ) \zeta ( 7 ) \zeta ( 8 )} \\ 
 A_{w_{\para{P}_{3} }} = &\frac{R^{7}}{\zeta ( 2 )^{2} \zeta ( 3 ) \zeta ( 4 ) \zeta ( 5 ) \zeta ( 6 ) \zeta ( 7 )}\\ 
 A_{w_{\para{P}_{4} }} = &\frac{R^{7}}{\zeta ( 2 )^{3} \zeta ( 3 )^{2} \zeta ( 4 ) \zeta ( 5 )} \\ 
 A_{w_{\para{P}_{5} }} = &\frac{R^{7}}{\zeta ( 2 )^{2} \zeta ( 3 )^{2} \zeta ( 4 )^{2} \zeta ( 5 )} \\
 A_{w_{\para{P}_{6} }} = &\frac{R^{7}}{\zeta ( 2 )^{2} \zeta ( 3 ) \zeta ( 4 ) \zeta ( 5 ) \zeta ( 6 ) \zeta ( 8 )}\\
 A_{w_{\para{P}_{7} }} = &\frac{R^{7}}{\zeta ( 2 )^{2} \zeta ( 5 ) \zeta ( 6 ) \zeta ( 8 ) \zeta ( 12 ) \zeta ( 9 )}\\
 A_{w_{\para{P}_{8} }} = &\frac{R^{7}}{\zeta ( 2 ) \zeta ( 6 ) \zeta ( 8 ) \zeta ( 10 ) \zeta ( 18 ) \zeta ( 12 ) \zeta ( 14 )}\\ 
  \end{align*} 
  where:
  \begin{align*}
w_{\para{P}_{1} } =&  w_{8}w_{7}w_{6}w_{5}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{8}w_{7}w_{6}w_{5}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{6}w_{5} w_{4}w_{3}w_{2}w_{4}w_{5}
 \\
& w_{6}w_{5}w_{4}w_{3}w_{2}w_{4}w_{5}w_{4}w_{3}w_{2}w_{4}w_{3}w_{2} \\ 
 w_{\para{P}_{2} } =&  w_{1}w_{3}w_{4}w_{5}w_{6}w_{7}w_{8}w_{1}w_{3}w_{4}w_{5}w_{6}w_{7}w_{1}w_{3}w_{4}w_{5}w_{6}w_{1}w_{3}w_{4}w_{5}w_{1}w_{3}w_{4}w_{1}w_{3}w_{1}\\
 w_{\para{P}_{3} } =&  w_{2}w_{4}w_{5}w_{6}w_{7}w_{8}w_{2}w_{4}w_{5}w_{6}w_{7}w_{2}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5}w_{2}w_{4}w_{2}w_{1} \\ 
 w_{\para{P}_{4} } =&  w_{5}w_{6}w_{7}w_{8}w_{5}w_{6}w_{7}w_{5}w_{6}w_{5}w_{1}w_{3}w_{2}w_{1} \\
 w_{\para{P}_{5} } =&  w_{6}w_{7}w_{8}w_{6}w_{7}w_{6}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{1}w_{3}w_{2}w_{1} \\ 
 w_{\para{P}_{6} } =&  w_{7}w_{8}w_{7}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{1}w_{3}w_{2}w_{1} \\ 
 w_{\para{P}_{7} } =&  w_{8}w_{1}w_{3}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}
 \\ & w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{1}w_{3}w_{2}w_{1} \\ 
 w_{\para{P}_{8} } =&  w_{7}w_{6}w_{5}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{1}w_{3}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{1}w_{3}w_{4}w_{5}w_{6}w_{2}w_{4} \\
 & w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{1}w_{3}w_{2}w_{1} \\ 
  \end{align*}
 \end{prop} 
 \newpage
 \begin{landscape}
 \begin{longtable}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
$ \para{P}_i $ & $ s $ & $ \para{P}_j $ & $ t $ & $ w $ & $\frac{h_4(\chi_t)}{h_4(\chi_s)}$ & $d_{\para{P}_i}(\chi_s)$ & $d_{\para{P}_j}(\chi_t)$ & $ d $ & $ \epsilon_s $ & $ \epsilon_t $ \\ \hline
$\para{P}_{1}$ & $ \frac{11}{46} $ & $\para{P}_{8}$ & $ \frac{5}{58} $ & $ w_{8}w_{7}w_{6}w_{5}w_{4}w_{3}w_{2}w_{4}w_{5}w_{6}w_{7}w_{8} $ & $\frac{\zeta ( 6 ) \zeta ( 2 )}{\zeta ( 7 ) \zeta ( 12 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 23 $ & $ 1 $ \\ \hline
$\para{P}_{2}$ & $ \frac{7}{34} $ & $\para{P}_{1}$ & $ \frac{7}{46} $ & $ w_{1}w_{3}w_{4}w_{5}w_{6}w_{7}w_{8} $ & $\frac{\zeta ( 2 )}{\zeta ( 8 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 578 $ & $ 46 $ \\ \hline
$\para{P}_{2}$ & $ \frac{5}{34} $ & $\para{P}_{7}$ & $ \frac{3}{38} $ & $ w_{7}w_{8}w_{6}w_{7}w_{5}w_{6}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 7 ) \zeta ( 8 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 578 $ & $ 19 $ \\ \hline
$\para{P}_{2}$ & $ \frac{11}{34} $ & $\para{P}_{8}$ & $ \frac{13}{58} $ & $ w_{8}w_{7}w_{6}w_{5}w_{4}w_{3}w_{1} $ & $\frac{\zeta ( 2 )}{\zeta ( 8 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 17 $ & $ 1 $ \\ \hline
$\para{P}_{3}$ & $ \frac{11}{26} $ & $\para{P}_{1}$ & $ \frac{19}{46} $ & $ w_{1} $ & $ 1 $ & $ 1 $ & $ 0 $ & $ 1 $ & $ 13 $ & $ 1 $ \\ \hline
$\para{P}_{3}$ & $ \frac{3}{26} $ & $\para{P}_{2}$ & $ \frac{3}{34} $ & $ w_{2}w_{4}w_{5}w_{6}w_{7}w_{8} $ & $\frac{\zeta ( 2 )}{\zeta ( 7 )}$ & $ 3 $ & $ 2 $ & $ 1 $ & $ 13182 $ & $ 1734 $ \\ \hline
$\para{P}_{3}$ & $ \frac{1}{26} $ & $\para{P}_{6}$ & $ 0 $ & $ w_{6}w_{7}w_{8}w_{5}w_{6}w_{7}w_{4}w_{5}w_{6}w_{2}w_{4}w_{5} $ & $\frac{\zeta ( 3 ) \zeta ( 2 )^{2}}{\zeta ( 5 ) \zeta ( 6 ) \zeta ( 7 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 26 $ & $ 1 $ \\ \hline
$\para{P}_{3}$ & $ \frac{5}{26} $ & $\para{P}_{7}$ & $ \frac{5}{38} $ & $ w_{7}w_{8}w_{6}w_{7}w_{5}w_{6}w_{4}w_{5}w_{2}w_{4} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 6 ) \zeta ( 7 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 338 $ & $ 38 $ \\ \hline
$\para{P}_{3}$ & $ \frac{9}{26} $ & $\para{P}_{8}$ & $ \frac{15}{58} $ & $ w_{8}w_{7}w_{6}w_{5}w_{4}w_{2} $ & $\frac{\zeta ( 2 )}{\zeta ( 7 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 13 $ & $ 1 $ \\ \hline
$\para{P}_{4}$ & $ \frac{7}{18} $ & $\para{P}_{1}$ & $ \frac{17}{46} $ & $ w_{1}w_{3} $ & $\frac{\zeta ( 2 )}{\zeta ( 3 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 81 $ & $ 23 $ \\ \hline
$\para{P}_{4}$ & $ \frac{7}{18} $ & $\para{P}_{2}$ & $ \frac{13}{34} $ & $ w_{2} $ & $ 1 $ & $ 2 $ & $ 1 $ & $ 1 $ & $ 81 $ & $ 17 $ \\ \hline
$\para{P}_{4}$ & $ \frac{5}{18} $ & $\para{P}_{3}$ & $ \frac{7}{26} $ & $ w_{3}w_{1} $ & $\frac{\zeta ( 2 )}{\zeta ( 3 )}$ & $ 3 $ & $ 2 $ & $ 1 $ & $ 1458 $ & $ 338 $ \\ \hline
$\para{P}_{4}$ & $ \frac{1}{18} $ & $\para{P}_{5}$ & $ \frac{1}{22} $ & $ w_{5}w_{6}w_{7}w_{8} $ & $\frac{\zeta ( 2 )}{\zeta ( 5 )}$ & $ 5 $ & $ 4 $ & $ 1 $ & $ 42515280 $ & $ 1756920 $ \\ \hline
$\para{P}_{4}$ & $ \frac{1}{6} $ & $\para{P}_{6}$ & $ \frac{1}{7} $ & $ w_{6}w_{7}w_{8}w_{5}w_{6}w_{7} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 4 ) \zeta ( 5 )}$ & $ 4 $ & $ 3 $ & $ 1 $ & $ 78732 $ & $ 16464 $ \\ \hline
$\para{P}_{4}$ & $ \frac{5}{18} $ & $\para{P}_{7}$ & $ \frac{9}{38} $ & $ w_{7}w_{8}w_{6}w_{7}w_{5}w_{6} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 4 ) \zeta ( 5 )}$ & $ 3 $ & $ 2 $ & $ 1 $ & $ 1458 $ & $ 722 $ \\ \hline
$\para{P}_{4}$ & $ \frac{7}{18} $ & $\para{P}_{8}$ & $ \frac{19}{58} $ & $ w_{8}w_{7}w_{6}w_{5} $ & $\frac{\zeta ( 2 )}{\zeta ( 5 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 81 $ & $ 29 $ \\ \hline
$\para{P}_{5}$ & $ \frac{7}{22} $ & $\para{P}_{1}$ & $ \frac{13}{46} $ & $ w_{1}w_{3}w_{4}w_{2} $ & $\frac{\zeta ( 2 )}{\zeta ( 5 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 121 $ & $ 23 $ \\ \hline
$\para{P}_{5}$ & $ \frac{5}{22} $ & $\para{P}_{2}$ & $ \frac{7}{34} $ & $ w_{2}w_{4}w_{3}w_{1} $ & $\frac{\zeta ( 2 )}{\zeta ( 5 )}$ & $ 3 $ & $ 2 $ & $ 1 $ & $ 2662 $ & $ 578 $ \\ \hline
$\para{P}_{5}$ & $ \frac{3}{22} $ & $\para{P}_{3}$ & $ \frac{3}{26} $ & $ w_{3}w_{4}w_{1}w_{3}w_{2}w_{4} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 4 ) \zeta ( 5 )}$ & $ 4 $ & $ 3 $ & $ 1 $ & $ 175692 $ & $ 13182 $ \\ \hline
$\para{P}_{5}$ & $ \frac{5}{22} $ & $\para{P}_{6}$ & $ \frac{3}{14} $ & $ w_{6}w_{7}w_{8} $ & $\frac{\zeta ( 2 )}{\zeta ( 4 )}$ & $ 3 $ & $ 2 $ & $ 1 $ & $ 2662 $ & $ 392 $ \\ \hline
$\para{P}_{5}$ & $ \frac{7}{22} $ & $\para{P}_{7}$ & $ \frac{11}{38} $ & $ w_{7}w_{8}w_{6}w_{7} $ & $\frac{\zeta ( 2 )^{2}}{\zeta ( 3 ) \zeta ( 4 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 121 $ & $ 19 $ \\ \hline
$\para{P}_{5}$ & $ \frac{9}{22} $ & $\para{P}_{8}$ & $ \frac{21}{58} $ & $ w_{8}w_{7}w_{6} $ & $\frac{\zeta ( 2 )}{\zeta ( 4 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 11 $ & $ 1 $ \\ \hline
$\para{P}_{6}$ & $ \frac{3}{14} $ & $\para{P}_{1}$ & $ \frac{7}{46} $ & $ w_{1}w_{3}w_{4}w_{5}w_{2}w_{4}w_{3}w_{1} $ & $\frac{\zeta ( 4 ) \zeta ( 2 )}{\zeta ( 5 ) \zeta ( 8 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 392 $ & $ 46 $ \\ \hline
$\para{P}_{6}$ & $ \frac{1}{14} $ & $\para{P}_{2}$ & $ \frac{1}{34} $ & $ w_{2}w_{4}w_{5}w_{3}w_{4}w_{1}w_{3}w_{2}w_{4}w_{5} $ & $\frac{\zeta ( 3 ) \zeta ( 2 )}{\zeta ( 6 ) \zeta ( 8 )}$ & $ 2 $ & $ 1 $ & $ 1 $ & $ 1176 $ & $ 34 $ \\ \hline
$\para{P}_{6}$ & $ \frac{5}{14} $ & $\para{P}_{7}$ & $ \frac{13}{38} $ & $ w_{7}w_{8} $ & $\frac{\zeta ( 2 )}{\zeta ( 3 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 14 $ & $ 1 $ \\ \hline
$\para{P}_{6}$ & $ \frac{3}{7} $ & $\para{P}_{8}$ & $ \frac{23}{58} $ & $ w_{8}w_{7} $ & $\frac{\zeta ( 2 )}{\zeta ( 3 )}$ & $ 1 $ & $ 0 $ & $ 1 $ & $ 14 $ & $ 1 $ \\ \hline
$\para{P}_{7}$ & $ \frac{17}{38} $ & $\para{P}_{8}$ & $ \frac{25}{58} $ & $ w_{8} $ & $ 1 $ & $ 1 $ & $ 0 $ & $ 1 $ & $ 19 $ & $ 1 $ \\ \hline
\end{longtable}
 \end{landscape}
 \begin{thm} 
Let $f^{0} \in I_{\para{P}_i}(s)$ be the normalized spherical section then:
\begin{enumerate} 
\item 
 $\leadingterm{-1}^{\para{P}_{1} } (f^{0},{\frac{11}{46}},g)=\frac{1}{23} \times \frac{R \zeta ( 6 ) \zeta ( 4 )}{\zeta ( 12 ) \zeta ( 14 ) \zeta ( 18 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{5}{58}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{2} } (f^{0},{\frac{7}{34}},g)=\frac{23}{289} \times \frac{R \zeta ( 5 ) \zeta ( 3 )}{\zeta ( 8 ) \zeta ( 12 ) \zeta ( 10 )} \times  \leadingterm{-1}^{\para{P}_{1} } (f^{0},{\frac{7}{46}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{2} } (f^{0},{\frac{5}{34}},g)=\frac{19}{578} \times \frac{R \zeta ( 4 ) \zeta ( 3 )}{\zeta ( 8 ) \zeta ( 9 ) \zeta ( 12 )} \times  \leadingterm{-1}^{\para{P}_{7} } (f^{0},{\frac{3}{38}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{2} } (f^{0},{\frac{11}{34}},g)=\frac{1}{17} \times \frac{R \zeta ( 7 ) \zeta ( 5 ) \zeta ( 4 ) \zeta ( 3 )}{\zeta ( 8 ) \zeta ( 14 ) \zeta ( 12 ) \zeta ( 18 ) \zeta ( 10 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{13}{58}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{3} } (f^{0},{\frac{11}{26}},g)=\frac{1}{13} \times \frac{R \zeta ( 5 ) \zeta ( 3 )}{\zeta ( 12 ) \zeta ( 10 ) \zeta ( 8 )} \times  \leadingterm{0}^{\para{P}_{1} } (f^{0},{\frac{19}{46}},g) \\ 
$\item 
 $\leadingterm{-3}^{\para{P}_{3} } (f^{0},{\frac{3}{26}},g)=\frac{289}{2197} \times \frac{R \zeta ( 2 )}{\zeta ( 7 ) \zeta ( 8 )} \times  \leadingterm{-2}^{\para{P}_{2} } (f^{0},{\frac{3}{34}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{3} } (f^{0},{\frac{1}{26}},g)=\frac{1}{26} \times \frac{R \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 6 ) \zeta ( 5 ) \zeta ( 8 )} \times  \leadingterm{0}^{\para{P}_{6} } (f^{0},{0},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{3} } (f^{0},{\frac{5}{26}},g)=\frac{19}{169} \times \frac{R \zeta ( 4 ) \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 6 ) \zeta ( 9 ) \zeta ( 12 ) \zeta ( 8 )} \times  \leadingterm{-1}^{\para{P}_{7} } (f^{0},{\frac{5}{38}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{3} } (f^{0},{\frac{9}{26}},g)=\frac{1}{13} \times \frac{R \zeta ( 5 ) \zeta ( 4 ) \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 14 ) \zeta ( 12 ) \zeta ( 18 ) \zeta ( 10 ) \zeta ( 8 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{15}{58}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{4} } (f^{0},{\frac{7}{18}},g)=\frac{23}{81} \times \frac{R \zeta ( 5 ) \zeta ( 3 ) \zeta ( 2 )^{2}}{\zeta ( 12 ) \zeta ( 10 ) \zeta ( 8 ) \zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-1}^{\para{P}_{1} } (f^{0},{\frac{17}{46}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{4} } (f^{0},{\frac{7}{18}},g)=\frac{17}{81} \times \frac{R \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 8 ) \zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-1}^{\para{P}_{2} } (f^{0},{\frac{13}{34}},g) \\ 
$\item 
 $\leadingterm{-3}^{\para{P}_{4} } (f^{0},{\frac{5}{18}},g)=\frac{169}{729} \times \frac{R \zeta ( 2 )}{\zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-2}^{\para{P}_{3} } (f^{0},{\frac{7}{26}},g) \\ 
$\item 
 $\leadingterm{-5}^{\para{P}_{4} } (f^{0},{\frac{1}{18}},g)=\frac{14641}{354294} \times \frac{R \zeta ( 2 )}{\zeta ( 5 ) \zeta ( 4 )} \times  \leadingterm{-4}^{\para{P}_{5} } (f^{0},{\frac{1}{22}},g) \\ 
$\item 
 $\leadingterm{-4}^{\para{P}_{4} } (f^{0},{\frac{1}{6}},g)=\frac{1372}{6561} \times \frac{R \zeta ( 3 ) \zeta ( 2 )^{2}}{\zeta ( 5 ) \zeta ( 4 ) \zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{-3}^{\para{P}_{6} } (f^{0},{\frac{1}{7}},g) \\ 
$\item 
 $\leadingterm{-3}^{\para{P}_{4} } (f^{0},{\frac{5}{18}},g)=\frac{361}{729} \times \frac{R \zeta ( 3 )^{2} \zeta ( 2 )^{2}}{\zeta ( 5 ) \zeta ( 9 ) \zeta ( 12 ) \zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{-2}^{\para{P}_{7} } (f^{0},{\frac{9}{38}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{4} } (f^{0},{\frac{7}{18}},g)=\frac{29}{81} \times \frac{R \zeta ( 4 ) \zeta ( 3 )^{2} \zeta ( 2 )^{2}}{\zeta ( 14 ) \zeta ( 12 ) \zeta ( 18 ) \zeta ( 10 ) \zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{-1}^{\para{P}_{8} } (f^{0},{\frac{19}{58}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{5} } (f^{0},{\frac{7}{22}},g)=\frac{23}{121} \times \frac{R \zeta ( 4 ) \zeta ( 3 )^{2} \zeta ( 2 )}{\zeta ( 12 ) \zeta ( 10 ) \zeta ( 8 ) \zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-1}^{\para{P}_{1} } (f^{0},{\frac{13}{46}},g) \\ 
$\item 
 $\leadingterm{-3}^{\para{P}_{5} } (f^{0},{\frac{5}{22}},g)=\frac{289}{1331} \times \frac{R \zeta ( 4 ) \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 5 ) \zeta ( 8 ) \zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-2}^{\para{P}_{2} } (f^{0},{\frac{7}{34}},g) \\ 
$\item 
 $\leadingterm{-4}^{\para{P}_{5} } (f^{0},{\frac{3}{22}},g)=\frac{2197}{29282} \times \frac{R \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 5 ) \zeta ( 7 ) \zeta ( 6 )} \times  \leadingterm{-3}^{\para{P}_{3} } (f^{0},{\frac{3}{26}},g) \\ 
$\item 
 $\leadingterm{-3}^{\para{P}_{5} } (f^{0},{\frac{5}{22}},g)=\frac{196}{1331} \times \frac{R \zeta ( 3 )}{\zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{-2}^{\para{P}_{6} } (f^{0},{\frac{3}{14}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{5} } (f^{0},{\frac{7}{22}},g)=\frac{19}{121} \times \frac{R \zeta ( 4 ) \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 9 ) \zeta ( 12 ) \zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{-1}^{\para{P}_{7} } (f^{0},{\frac{11}{38}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{5} } (f^{0},{\frac{9}{22}},g)=\frac{1}{11} \times \frac{R \zeta ( 5 ) \zeta ( 4 ) \zeta ( 3 )^{2} \zeta ( 2 )}{\zeta ( 14 ) \zeta ( 12 ) \zeta ( 18 ) \zeta ( 10 ) \zeta ( 8 ) \zeta ( 6 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{21}{58}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{6} } (f^{0},{\frac{3}{14}},g)=\frac{23}{196} \times \frac{R \zeta ( 4 ) \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 8 ) \zeta ( 12 ) \zeta ( 10 ) \zeta ( 7 )} \times  \leadingterm{-1}^{\para{P}_{1} } (f^{0},{\frac{7}{46}},g) \\ 
$\item 
 $\leadingterm{-2}^{\para{P}_{6} } (f^{0},{\frac{1}{14}},g)=\frac{17}{588} \times \frac{R \zeta ( 3 ) \zeta ( 2 )}{\zeta ( 8 ) \zeta ( 6 ) \zeta ( 7 )} \times  \leadingterm{-1}^{\para{P}_{2} } (f^{0},{\frac{1}{34}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{6} } (f^{0},{\frac{5}{14}},g)=\frac{1}{14} \times \frac{R \zeta ( 4 )}{\zeta ( 9 ) \zeta ( 12 )} \times  \leadingterm{0}^{\para{P}_{7} } (f^{0},{\frac{13}{38}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{6} } (f^{0},{\frac{3}{7}},g)=\frac{1}{14} \times \frac{R \zeta ( 5 ) \zeta ( 4 ) \zeta ( 2 )}{\zeta ( 14 ) \zeta ( 12 ) \zeta ( 18 ) \zeta ( 10 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{23}{58}},g) \\ 
$\item 
 $\leadingterm{-1}^{\para{P}_{7} } (f^{0},{\frac{17}{38}},g)=\frac{1}{19} \times \frac{R \zeta ( 9 ) \zeta ( 5 )}{\zeta ( 14 ) \zeta ( 18 ) \zeta ( 10 )} \times  \leadingterm{0}^{\para{P}_{8} } (f^{0},{\frac{25}{58}},g) \\ 
$\end{enumerate} 
\end{thm} 


\begin{figure}[H]
\begin{center}
\begin{tikzpicture}[thin,scale=2]
\tikzset{
  text style/.style={
    sloped, % the text will be parallel to the connection 
    text=black,
    font=\tiny,
    above
  }
}
%nodes
\matrix (m) [matrix of math nodes, row sep=1em, column sep=3em]
    { 		
    %first row
       |[name=p11146]| \text{I}_{\para{P}_1}(\frac{11}{46})
        &  |[name=p8558]| \text{I}_{\para{P}_8}(\frac{5}{58})
       & &
		|[name=p21134]| \text{I}_{\para{P}_2}(\frac{11}{34})
       &  |[name=p81358]| \text{I}_{\para{P}_8}(\frac{13}{58})
      \\
       |[name=p3926]| \text{I}_{\para{P}_3}(\frac{9}{26})
              &  |[name=p81558]| \text{I}_{\para{P}_8}(\frac{15}{58})
             & &
        |[name=p6514]| \text{I}_{\para{P}_6}(\frac{5}{14})
              &  |[name=p71338]| \text{I}_{\para{P}_7}(\frac{13}{38})
           
\\
		|[name=p5922]| \text{I}_{\para{P}_5}(\frac{9}{22})
       &  |[name=p82158]| \text{I}_{\para{P}_8}(\frac{21}{58})
& &
      |[name=p637]| \text{I}_{\para{P}_6}(\frac{3}{7})
       &  |[name=p82358]| \text{I}_{\para{P}_8}(\frac{23}{58})
\\
|[name=p71738]| \text{I}_{\para{P}_7}(\frac{17}{38})
      &  |[name=p82558]| \text{I}_{\para{P}_8}(\frac{25}{58})
& &
|[name=p2534]| \text{I}_{\para{P}_2}(\frac{5}{34})
      &  |[name=p7338]| \text{I}_{\para{P}_7}(\frac{3}{38})
\\
|[name=p3526]| \text{I}_{\para{P}_3}(\frac{5}{26})
      &  |[name=p7538]| \text{I}_{\para{P}_7}(\frac{5}{38})
%|[name=p5722]| \text{I}_{\para{P}_5}(\frac{7}{22})
%      &  |[name=p71138]| \text{I}_{\para{P}_7}(\frac{11}{38})
& & 
|[name=p31126]| \text{I}_{\para{P}_3}(\frac{11}{26})
        &  |[name=p11946]| \text{I}_{\para{P}_1}(\frac{19}{46})
\\
|[name=p3126]| \text{I}_{\para{P}_3}(\frac{1}{26})
      &  |[name=p60]| \text{I}_{\para{P}_6}(0)
& & 
|[name=p416]| \text{I}_{\para{P}_4}(\frac{1}{6})
      &  |[name=p617]| \text{I}_{\para{P}_6}(\frac{1}{7})
\\
|[name=p6114]| \text{I}_{\para{P}6}(\frac{1}{14})
      &  |[name=p2134]| \text{I}_{\para{P}_2}(\frac{1}{34})
& & 
|[name=p4118]| \text{I}_{\para{P}_4}(\frac{1}{18})
      &  |[name=p5122]| \text{I}_{\para{P}_5}(\frac{1}{22})
\\

& 
|[name=p5322]| \text{I}_{\para{P}_5}(\frac{3}{22})
      &  |[name=p3326]| \text{I}_{\para{P}_3}(\frac{3}{26})
      &
      |[name=p2334]| \text{I}_{\para{P}_2}(\frac{3}{34})
      \\
&
  |[name=p11746]| \text{I}_{\para{P}_1}(\frac{17}{46})
 & & |[name=p2734]| \text{I}_{\para{P}_2}(\frac{7}{34})
\\
  |[name=p4718]| \text{I}_{\para{P}_4}(\frac{7}{18})
&
  |[name=p21334]| \text{I}_{\para{P}_2}(\frac{13}{34})
 &  |[name=p5522]| \text{I}_{\para{P}_5}(\frac{5}{22}) & &
 |[name=p1746]| \text{I}_{\para{P}_1}(\frac{7}{46})
 \\
 &
     |[name=p81958]| \text{I}_{\para{P}_8}(\frac{19}{58})
  & 

  & |[name=p6314]| \text{I}_{\para{P}_6}(\frac{3}{14})
\\

&
|[name=p3726]| \text{I}_{\para{P}_3}(\frac{7}{26})
  & 
&
  & |[name=p11346]| \text{I}_{\para{P}_1}(\frac{13}{46})
\\
|[name=p4518]| \text{I}_{\para{P}_4}(\frac{5}{18})
  & 
&
  & |[name=p5722]| \text{I}_{\para{P}_5}(\frac{7}{22})
  
  \\
  
  &
  |[name=p7938]| \text{I}_{\para{P}_7}(\frac{9}{38})
    & 
  &
    & |[name=p71138]| \text{I}_{\para{P}_7}(\frac{11}{38})
  
    \\};

\draw[->]      
(p11146)  edge [-]
node[text style,above]{}  (p8558)

(p21134)  edge [-]
node[text style,above]{}  (p81358)

(p3926)  edge [-]
node[text style,above]{}  (p81558)

(p4718)  edge [-]
node[text style,above]{}  (p81958)

(p5922)  edge [-]
node[text style,above]{}  (p82158)

(p637)  edge [-]
node[text style,above]{}  (p82358)

(p71738)  edge [-]
node[text style,above]{}  (p82558)

(p2534)  edge [-]
node[text style,above]{}  (p7338)
(p3526)  edge [-]
node[text style,above]{}  (p7538)

(p4518)  edge [-]
node[text style,above]{}  (p7938)

(p5722)  edge [-]
node[text style,above]{}  (p71138)

(p6514)  edge [-]
node[text style,above]{}  (p71338)

(p3126)  edge [-]
node[text style,above]{}  (p60)

(p416)  edge [-]
node[text style,above]{}  (p617)

(p6114)  edge [-]
node[text style,above]{}  (p2134)

(p4118)  edge [-]
node[text style,above]{}  (p5122)

(p4718)  edge [-]
node[text style,above]{}  (p11746)

(p4718)  edge [-]
node[text style,above]{}  (p21334)
(p4518)  edge [-]
node[text style,above]{}  (p3726)
(p5722)  edge [-]
node[text style,above]{}  (p71138)

(p5722)  edge [-]
node[text style,above]{}  (p11346)

(p5322)  edge [-]
node[text style,above]{}  (p3326)
(p3326)  edge [-]
node[text style,above]{}  (p2334)

(p5522)  edge [-]
node[text style,above]{}  (p2734)
(p5522)  edge [-]
node[text style,above]{}  (p6314)
(p2734)  edge [-]
node[text style,above]{}  (p1746)
(p6314)  edge [-]
node[text style,above]{}  (p1746)

(p31126)  edge [-]
node[text style,above]{}  (p11946)

;
\end{tikzpicture}
\label{digram:E8s}
\end{center}
\end{figure}


==> Chapters/new/new_techinal_lemma.tex <==
\chapter{Find the constant} % Main chapter title

\label{ch:Technical lemmas} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

\lhead{Chapter \ref{ch:Technical lemmas}. \emph{Find the constant}} % Change X to a consecutive number; this is for the header on each page - perhaps a shortened title
In this chapter we give an explicit formula for the constant that appears in Theorem (\ref{EiseConst}).
This will be done by  proving some technical lemmas regarding to $E_{\para{B}}^{\#}(\chi,g)$.
During the all chapter $\chi$ will be an unramified character of $T$, and $w$ will be some element in $\weyl{G}$. 
Let fix some notations:
\begin{align*}
N_{\epsilon}(\chi)&=\{\alpha \in \Phi^{+} \: : \left \langle \chi ,\check{\alpha} \right \rangle =\epsilon\} &
B_{\epsilon}(\chi)&=\{\alpha \in \Phi \: : \left \langle \chi ,\check{\alpha} \right \rangle =\epsilon\} \\
B_{\epsilon_1,\epsilon_2,\dots \epsilon_n}(\chi)&=\cup_{i}^{n}B_{\epsilon_i}(\chi)
& N_{\epsilon_1,\epsilon_2,\dots \epsilon_n}(\chi)&=\cup_{i}^{n}N_{\epsilon_i}(\chi)\\
l_{\alpha}^{+}(\chi)&=(\left \langle \chi ,\check{\alpha} \right \rangle+1) &
l_{\alpha}^{-}(\chi)&=(\left \langle \chi ,\check{\alpha} \right \rangle-1) \\
h_1(\chi) &=\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)
&
h_2(\chi)&=\prod_{\alpha \in \Phi}l_{\alpha}^{+}(\chi)
\\
h_3(\chi) &=\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi \\
\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}
l_{\alpha}^{+}(\chi)
&
h_4(\chi) &=\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\alpha}^{+}(\chi)) 
\\
\mathcal{F}_{\alpha}^{+}&=\{\chi \in \mathfrak{a}^{\ast}_{\mathbb{C}} \: : l_{\alpha}^{+}(\chi)=0 \} &
\mathcal{F}_{\alpha}^{-}&=\{\chi \in \mathfrak{a}^{\ast}_{\mathbb{C}} \: : l_{\alpha}^{-}(\chi)=0 \}
\end{align*}
For a maximal parabolic subgroup $\para{P}_i$ let $b_{ii} \in \mathbb{C} $ such that $\delta_{\para{P}_i}=b_{ii}\fundamental{i}$
\begin{lemm}[Lemma-T1]\label{Lemma-T1}
Let $\chi$ be an unramified character of $T$. For every $\epsilon\in \mathbb{C}$ and $\weylelement{} \in \weyl{G} $ it holds that:
\begin{enumerate}
\item\label{Lemma-T1-2}
	$B_{\epsilon}(\weylelement{}\chi)=\weylelement{}B_{\epsilon}(\chi)$
\item\label{Lemma-T1-1}
$B_{\epsilon}(\chi)=-B_{-\epsilon}(\chi)$

\end{enumerate}
\end{lemm}
\begin{proof}
\begin{align*}
\alpha \in B_{\epsilon}(\weylelement{}\chi) & \iff \left \langle \weylelement{}\chi ,\check{\alpha} \right \rangle =\epsilon & \iff \left \langle \chi ,\weylelement{}^{-1}\check{\alpha} \right \rangle =\epsilon & \iff \weylelement{}^{-1} \alpha \in B_{\epsilon}(\chi) \iff \alpha \in \weylelement{}B_{\epsilon}(\chi)
\end{align*}
In a similar way we get the second statement.
\end{proof}
\begin{lemm}\label{Size_Lemma}
For every $\chi$ and $\weylelement{} \in \weyl{G}$ it holds that $|N_{\pm1}(\chi)| = |N_{\pm1}(\weylelement{}\chi)|$ and $|N_{0}(\chi)|=|N_{0}(\weylelement{}\chi)|$
\end{lemm}
\iffalse
\begin{proof}
In order to show this it enough to show that we have injective maps between to two sets. 
We define $H_5: \: N_{\pm1}(\weylelement{}\chi) \rightarrow N_{\pm1}(\chi)$ by the following rule:
$$H_5(\alpha) =
\begin{cases}
\weylelement{}^{-1}\alpha  & \text{if }  \weylelement{}^{-1}\alpha>0 \\
-\weylelement{}^{-1}\alpha  & \text{if }  \weylelement{}^{-1}\alpha<0 
\end{cases}
$$
It easy to see that this map is injective.
The same map works for the other direction.

The same argument works for the other direction.
\end{proof}
\fi
\begin{proof}

Note that
\begin{align*}
 B_{\epsilon}(\chi) &= \{ \alpha \in \Phi \: : \: \inner{\chi,\check{\alpha}} = \epsilon \} \\
 &= \{ \alpha \in \Phi^{+} \: : \: \inner{\chi,\check{\alpha}} = \epsilon \} \cup 
 \{ \alpha \in \Phi^{-} \: : \: \inner{\chi,\check{\alpha}} = \epsilon \} \\
 &= N_{\epsilon}(\chi) \cup \{ \alpha \in \Phi^{+} \: : \: \inner{\chi,\check{\alpha}} = -\epsilon \} \\
 &= N_{\epsilon}(\chi) \cup  - N_{-\epsilon}(\chi)
 \end{align*}
 Moreover, if $\epsilon \neq 0$ it holds that $N_{\epsilon}(\chi) \cap -N_{-\epsilon}(\chi) =\emptyset $.
 By  item \ref{Lemma-T1-1} of Lemma (\ref{Lemma-T1}) we know that 
 $B_{1}(\weylelement{}\chi)=\weylelement{} B_{1}(\chi)$ since $\weylelement{}$ is injective we are done. 
 
Note that $B_{0}(\chi)= N_{0}(\chi) \cup -N_{0}(\chi)$. Moreover, $|N_{0}(\chi) | = |-N_{0}(\chi)|$ then by the same argument as in the first part we are done.
\end{proof}
\begin{cor}\label{cor_1}
With the same notation as above it holds that :
$$|N_{1}(\chi)| - | N_{-1} (\weylelement{}\chi) | = |N_{1}(\weylelement{}\chi)| -
|N_{-1}(\chi)|$$
\end{cor}
\begin{lemm}[Lemma-T2] \label{Lemma-T2}
For every $\chi$ it holds that 
$h_1(\chi)= (-1)^{|\Phi^{+}|}h_2(\chi)$
\end{lemm}
\begin{proof}
\begin{align*}
h_2(\chi)&= \prod_{\alpha \in \Phi}l_{\alpha}^{+}(\chi) \\
&=\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\alpha \in \Phi^{-}}l_{\alpha}^{+}(\chi)
\\
&=\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{-\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\\
%&=\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
%\prod_{-\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)\\
&=
\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\beta \in \Phi^{+}}l_{-\beta}^{+}(\chi)\\
&=
\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\beta \in \Phi^{+}}
(\left \langle \chi ,-\check{\beta} \right \rangle+1) \\
&=
\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\beta \in \Phi^{+}}
(-\left \langle \chi ,\check{\beta} \right \rangle+1) \\
&=(-1)^{|\Phi^{+}|} \times 
\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\beta \in \Phi^{+}}
(\left \langle \chi ,\check{\beta} \right \rangle-1) \\
&=(-1)^{|\Phi^{+}|} \times 
\prod_{\alpha \in \Phi^{+}}l_{\alpha}^{+}(\chi)
\prod_{\beta \in \Phi^{+}}
l_{\beta}^{-}(\chi) \\
&=(-1)^{|\Phi^{+}|} \times h_1(\chi)
\end{align*}
\end{proof}

\begin{lemm}[Lemma-T3] \label{Lemma-T3}
The function $h_2(\chi)$ is $W$ -invariant.
\end{lemm}
\begin{proof}
It is clear.
\end{proof}

\begin{lemm}
[Lemma -T4] \label{Lemma-T4}
$h_3(\chi)=h_3(\weylelement{}\chi)$.
\end{lemm}
\begin{proof}
\begin{align*}
h_3(\weylelement{}\chi)&=
 \prod_{\tiny {\begin{aligned}
 \alpha \in \Phi \\
 \alpha \not \in B_{\pm1,0}(\weylelement{}\chi)
 \end{aligned}}}
 l_{\alpha}^{+}(\weylelement{}\chi)=
  \prod_{\tiny {\begin{aligned}
  \alpha \in \Phi \\
  \alpha \not \in \weylelement{}B_{\pm1,0}(\chi)
  \end{aligned}}}
  l_{\weylelement{}^{-1}\alpha}^{+}(\chi) \\
  &=
    \prod_{\tiny {\begin{aligned}
    \alpha \in \Phi \\
    \weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)
    \end{aligned}}}
    l_{\weylelement{}^{-1}\alpha}^{+}(\chi) =
    \prod_{\tiny {\begin{aligned}
        \weylelement{}\beta \in \Phi \\
        \beta \not \in B_{\pm1,0}(\chi)
        \end{aligned}}}
        l_{\beta}^{+}(\chi)\\
	&=  
	    \prod_{\tiny {\begin{aligned}
	        \beta \in \weylelement{}^{-1}\Phi \\
	        \beta \not \in B_{\pm1,0}(\chi)
	        \end{aligned}}}
	        l_{\beta}^{+}(\chi)
=
	    \prod_{\tiny {\begin{aligned}
	        \beta \in \Phi \\
	        \beta \not \in B_{\pm1,0}(\chi)
	        \end{aligned}}}
	        l_{\beta}^{+}(\chi)=
	h_3(\chi)
\end{align*}
\end{proof}
\begin{lemm}[Lemma-T5] \label{Lemma-T5}
Let $\chi$ be character such that $h_4(\chi) \neq 0 $. Then $$\frac{h_4(\weylelement{}\chi)}{h_4(\chi)}= \prod_{\tiny {\begin{aligned}
\alpha \in \Phi^{+} \\
\alpha \not \in B_{\pm 1,0}(\chi)\\
\weylelement{}\alpha <0
\end{aligned}}}
\frac{
\zeta (\left \langle \chi ,\check{\alpha} \right \rangle)
}{\zeta(
\left \langle \chi ,\check{\alpha} \right \rangle+1)
}$$
\end{lemm}
\begin{proof}
\begin{align*}
h_4(\weylelement{}\chi) &=\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\alpha \not \in B_{\pm1,0}(\weylelement{}\chi)\\
\end{aligned}}}\zeta(l_{\alpha}^{+}(\weylelement{}\chi)) =
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\alpha \not \in \weylelement{}B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi)) \\
=& 
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))=
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha >0\\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))
\times 
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha <0\\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))\\
=&
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha >0\\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))
\times 
\prod_{\tiny{
\begin{aligned}
\weylelement{}\beta \in \Phi^{+} \\
\beta <0\\
\beta \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\beta}^{+}(\chi))\\
=&
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha >0\\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))
\times 
\prod_{\tiny{
\begin{aligned}
\weylelement{}\beta \in \Phi^{+} \\
-\beta >0\\
\beta \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\beta}^{+}(\chi))\\
=&
\prod_{\tiny{
\begin{aligned}
\alpha \in \Phi^{+} \\
\weylelement{}^{-1}\alpha >0\\
\weylelement{}^{-1}\alpha \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\weylelement{}^{-1}\alpha}^{+}(\chi))
\times 
\prod_{\tiny{
\begin{aligned}
\weylelement{}\gamma \in \Phi^{-} \\
\gamma >0\\
\gamma \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{-\gamma}^{+}(\chi))\\
=&
\prod_{\tiny{
\begin{aligned}
\weylelement{}\gamma \in \Phi^{+} \\
\gamma >0\\
\gamma \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(l_{\gamma}^{+}(\chi))
\times 
\prod_{\tiny{
\begin{aligned}
\weylelement{}\gamma \in \Phi^{-} \\
\gamma >0\\
\gamma \not \in B_{\pm1,0}(\chi)\\
\end{aligned}}}\zeta(
\left \langle \chi ,\check{\gamma} \right \rangle)
\\
\end{align*}
Now the Lemma  follows.
\end{proof}

Note that 
\begin{align*}
\prod_{\alpha \in B_{1}(\chi)} l_{\alpha}^{+}(\chi) &=2^{ |N_1(\chi)| + |N_{-1}(\chi)|} \\
\prod_{\alpha \in B_{-1}(\chi)} l_{\alpha}^{+}(\chi) &=(-1)^{|N_{1}(\chi)|} \prod_{\alpha \in N_{-1}(\chi)} l_{\alpha}^{+}(\chi) \times \prod_{\alpha \in N_{1}(\chi)} l_{\alpha}^{-}(\chi)
\end{align*}
\begin{lemm}
Let  $\chi$ be a character then Ikeda normalized factor can be written as :
\begin{align}
\prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)=&(-1)^{|\Phi^{+}|+|N_{1}(\chi)|} \times h_3(\chi) \times h_4(\chi) \\
&\times 
\prod_{\tiny \begin{aligned}
	\gamma  \in N_{-1}(\chi)
	\end{aligned}}
\zeta(l_{\gamma}^{+}(\chi))l_{\gamma}^{+}(\chi)  \\
&\times \prod_{\tiny \begin{aligned}
	\gamma  \in N_{1}(\chi)
	\end{aligned}}
l_{\gamma}^{-}(\chi) 
\times \prod_{\tiny \begin{aligned}
	\gamma  \in N_{0}(\chi)
	\end{aligned}}
\zeta(l_{\gamma}^{+}(\chi) )
\\
& \times
\zeta(2)^{|N_1(\chi)|} \times 
(2)^{|N_{1}(\chi)| + |N_{-1}(\chi)|}
\end{align}
\end{lemm}
\begin{proof}
\iffalse
\begin{align*}
\prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)=& h_1(\chi) \times \prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi)) \\
=&(-1)^{|\Phi^{+}|}\prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi)) \times h_2(\chi)\\
=&(-1)^{|\Phi^{+}|}\times \prod_{\alpha \in B_{\pm1,0}(\chi)}l_{\alpha}^{+}(\chi) \times h_3(\chi)\times \prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi))\\
=& (-1)^{|\Phi^{+}|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in B_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\alpha < 0 \\
\alpha  \in B_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in B_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\alpha < 0 \\
\alpha  \in B_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in B_{0}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) \\
=& (-1)^{|\Phi^{+}|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
-\alpha > 0 \\
\alpha  \in B_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
-\alpha > 0 \\
\alpha  \in B_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\\
=& (-1)^{|\Phi^{+}|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma > 0 \\
-\gamma  \in B_{1}(\chi)
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma > 0 \\
-\gamma  \in B_{-1}(\chi)
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
=& (-1)^{|\Phi^{+}|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma > 0 \\
\gamma  \in B_{-1}(\chi)
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma > 0 \\
\gamma  \in B_{1}(\chi)
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
=& (-1)^{|\Phi^{+}|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma \in N_{-1}(\chi) \\
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma  \in N_{1}(\chi)
\end{aligned}}
l_{-\gamma}^{+}(\chi) 
\\
=& (-1)^{|\Phi^{+}|+|N_1(\chi)|+|N_{-1}(\chi)|} h_3(\chi) h_4(\chi) \times \prod_{\tiny \begin{aligned}
\alpha > 0 \\
\alpha  \in N_{\pm1,0}(\chi)
\end{aligned}}\zeta(l_{\alpha}^{+}(\chi)) \\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma \in N_{-1}(\chi) \\
\end{aligned}}
l_{\gamma}^{-}(\chi) 
\\
&\times 
\prod_{\tiny \begin{aligned}
\alpha  \in N_{-1}(\chi)
\end{aligned}}
l_{\alpha}^{+}(\chi) 
\times 
\prod_{\tiny \begin{aligned}
\gamma  \in N_{1}(\chi)
\end{aligned}}
l_{\gamma}^{-}(\chi) 
\\
=&(-1)^{|\Phi^{+}|+|N_{1}(\chi)|} \times h_3(\chi) \times h_4(\chi) \\
&\times 
\prod_{\tiny \begin{aligned}
\gamma  \in N_{-1}(\chi)
\end{aligned}}
\zeta(l_{\gamma}^{+}(\chi))l_{\gamma}^{+}(\chi)  \\
&\times \prod_{\tiny \begin{aligned}
\gamma  \in N_{1}(\chi)
\end{aligned}}
l_{\gamma}^{-}(\chi) 
\times \prod_{\tiny \begin{aligned}
\gamma  \in N_{0}(\chi)
\end{aligned}}
\zeta(l_{\gamma}^{+}(\chi) )
\\
& \times
\zeta(2)^{|N_1(\chi)|} \times 
(2)^{|N_{1}(\chi)| + |N_{-1}(\chi)|}
\end{align*}
\fi
\begin{align*}
\prod_{\alpha\in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi) =& 
h_1(\chi) \times \prod_{\alpha \in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi)) \\
\overset{\ref{Lemma-T2}}{=}&(-1)^{|\Phi^{+}|} \times 
h_2(\chi) \times
\prod_{
\alpha \in N_{\pm1,0}(\chi)
}
\zeta(l_{\alpha}^{+}(\chi))
\times 
\prod_{
		0<\alpha \not \in N_{\pm1,0}(\chi)
	}
\zeta(l_{\alpha}^{+}(\chi)) \\
=&(-1)^{|\Phi^{+}|} \times 
h_2(\chi) \times h_4(\chi)
\prod_{
	\alpha \in N_{\pm1,0}(\chi)
}
\zeta(l_{\alpha}^{+}(\chi))
\times 
\prod_{
	\alpha  \in B_{\pm1,0}(\chi)
}
l_{\alpha}^{+}(\chi) \\
=&(-1)^{|\Phi^{+}|} \times h_3(\chi) \times h_4(\chi) \times 
\prod_{\alpha \in N_{\pm1,0}}\zeta(l_{\alpha}^{+}(\chi))\\
&\times   \prod_{\alpha \in B_{1}(\chi)} l_{\alpha}^{+}(\chi) \times 
\prod_{\alpha \in B_{-1}(\chi)} l_{\alpha}^{+}(\chi)
\times 
\prod_{\alpha \in B_{0}(\chi)} l_{\alpha}^{+}(\chi) \\
=&(-1)^{|\Phi^{+}|+ |N_{1}(\chi)|}
\times  2^{|N_1(\chi)| +|N_{-1}(\chi)|}
\times \zeta(2)^{|N_1(\chi)|}
\times h_3(\chi) \times h_4(\chi) \\
&\times \prod_{\alpha \in N_{-1}(\chi)}
\zeta(l_{\alpha}^{+}(\chi)) l_{\alpha}^{+}(\chi)
\\
&\times 
 \prod_{\alpha \in N_{0}(\chi)}
 \zeta(l_{\alpha}^{+}(\chi))
\times  \prod_{\alpha \in N_{1}(\chi)} l_{\alpha}^{-}(\chi)
\end{align*}
\end{proof}
\begin{lemm}\label{new_tech_lemma}
Let $\para{P}=\para{P}_i$ be a maximal parabolic subgroup. Let 
$b_{ii} \in \mathbb{C}$ such that $\delta_{\para{P}}= b_{ii}\fundamental{i}$ then for 
$\chi_{s} = \delta_{\para{P}}^{s- \frac{1}{2}}\otimes \delta_{\para{B}}^{
\frac{1}{2}}$  and for every $\alpha \in \Phi^{+}$ is holds that there exists $a,m \in \mathbb{R}$ such that
$$l_{\alpha}^{+}(\chi_s) = as+m.$$ 
\end{lemm}
\begin{proof}
For $\alpha  \in \Phi^{+}$  we write  $\check{\alpha} = \sum_{j=1}^{n}n_{j}^{(\check{\alpha})}\check{\alpha}_{j}$ then:
\begin{align*}
\inner{\chi_s,\check{\alpha}} &= \inner{\delta_{\para{P}}^{s -\frac{1}{2}},\check{\alpha}} + \inner{\delta_{\para{B}}^{\frac{1}{2}},\check{\alpha}}\\
&= (s-\frac{1}{2})\inner{\delta_{\para{P}},\check{\alpha}} + \inner{ \sum_{k=1}^{n}\fundamental{k},\sum_{j=1}^{n}n_{j}^{(\check{\alpha})}\check{\alpha}_{j}} \\
&=b_{ii}(s-\frac{1}{2})\inner{\fundamental{i}, \sum_{j=1}^{n}n_{j}^{(\check{\alpha})}\check{\alpha}_{j}}+ \sum_{j=1}^{n} n_{j}^{(\check{\alpha})}\\
&= b_{ii}n_{i}^{(\check{\alpha})}(s-\frac{1}{2}) + \sum_{j=1}^{n} n_{j}^{(\check{\alpha})}
\end{align*}
Hence $$l_{\alpha}^{+}(\chi_s) = b_{ii}n_{i}^{(\check{\alpha})}s
+ \sum_{j=1}^{n} n_{j}^{(\check{\alpha})} + 1 -\frac{b_{ii} n_{i}^{(\check{\alpha})} }{2}
$$

\end{proof}
Now we will explore each term in the normalized Ikeda factor: 

\begin{lemm}\label{Corollary-1}
Let $\para{P}=\para{P}_i$ be a maximal parabolic subgroup of $G$. Let $b_{ii} \in \mathbb{C}$ such that $\delta_{\para{P}}=b_{ii} \fundamental{i}$. 
 Let $\chi_{s_0}= \delta_{\para{P}}^{s_{0}-\frac{1}{2}} \otimes \delta_{\para{B}}^{\frac{1}{2}}$. 
 For every $\alpha \in \Phi$ we write 
$ \check{\alpha } = \sum_{j=1}^{n}n_{j}^{(\check{\alpha})}\check{\alpha}_j$.
 Then 
\begin{enumerate}
	\item
	$\prod_{\alpha \in N_{-1}(\chi_{s_0})} \zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi) =(-R)^{|N_{-1}(\chi_{s_0})|}$ where $R=\operatorname{Res} _{s=1}\zeta(s)$
	\item
	The leading term of  $$H(s) =\prod_{\alpha \in N_{0}(\chi_{s_{0}})}\zeta(l_{\alpha}^{+}(\chi_{s})) \times \prod_{\tiny{
			\begin{aligned}
			\alpha \in N_{1}(\chi_{s_0}) \\
			\alpha \not \in \Delta_{\para{P}}\\
			\end{aligned}}}
		l_{\alpha}^{-}(\chi_{s})$$
		around $s=s_0$ is equal to 
		  $\epsilon_{s_0} \times R^{|N_{0}(\chi_{s_0})|}	\times (s-s_0)^{ |N_{1}(\chi_{s_0})| - |N_{0}(\chi_{s_0})|-(n-1)}$
		
\iffalse		
\begin{align*}
\prod_{\alpha \in N_{0}(\chi_{s_0})}\zeta(l_{\alpha}^{+}(\chi_{s_0})) \times \prod_{\tiny{
		\begin{aligned}
		\alpha \in N_{1}(\chi _{s_0}) \\
		\alpha \not \in \Delta_{\para{P}}\\
		\end{aligned}}}
	l_{\alpha}^{+}(\chi_{s_0}) =&\epsilon_{s_0} \times R^{|N_{0}(\chi_{s_0})|}	\times 0^{ |N_{1}(\chi_{s_0})| - |N_{0}(\chi)|-(n-1)}
\end{align*}
\fi
where 
\begin{align*}
\epsilon_{s_0} =&
	b_{ii}^{|N_1(\chi_{s_0})| - |N_0(\chi_{s_0})|-(n-1)}
	\times
	\prod_{
\alpha \in N_{0}(\chi_{s_0})
	}\frac{1}{n_{i}^{(\check{\alpha})}
	}
	\times
	\prod_{
			\alpha \in N_{1}(\chi_{s_0}) 	
		}{n_{i}^{(\check{\alpha})}}
	\end{align*}
\end{enumerate}
\begin{proof}
\begin{enumerate}
\item
It will be enough to show that if $\alpha \in N_{-1}(\chi_{s_0})$ then $$\zeta(l_{\alpha}^{+}(\chi_{s_0}))
l_{\alpha}^{+}(\chi_{s_0}) = -R.$$
But it is just the residue of $\zeta(s)$ at $s=0$ so we are done.
\item
Note that $H(s)$ is a meromorphic function (it is a product of such functions) therefore it admits a Laurent expansion around $s=s_0$. 
For every $\alpha \in N_{0}(\chi_{s_0})$ the element 
$\zeta(l_{\alpha}^{+}(\chi_s))$  can be written by Lemma (\ref{new_tech_lemma}) as $\zeta(F(s,\alpha))$ where 
$$F(s,\alpha)=b_{ii}n_{i}^{(\check{\alpha})}s+ m(\alpha).$$
By definition  $F(s_0,\alpha)=1$ therefore $\zeta(F(s,\alpha))$ admits a simple pole at $s=s_0$. The  Laurent expansion of $\zeta(F(s,\alpha))$ around $s_0$ is 
$$\zeta(F(s,\alpha)) = \sum_{j=-1}^{\infty} a_j(F(s,\alpha)-1)^i$$
where $a_{-1}=R$. 
Moreover,
\begin{align*}
F(s,\alpha)-1 &= F(s,\alpha)- F(s_0,\alpha) \\
&= b_{ii}n_{i}^{(\check{\alpha})}s+ m(\alpha) - ( b_{ii}n_{i}^{(\check{\alpha})}s_0+ m(\alpha)) \\
&= b_{ii}n_{i}^{(\check{\alpha})}(s-s_0)
\end{align*}
Therefore 
$$\zeta(F(s,\alpha))= \sum_{j=-1}^{\infty} a_j(b_{ii}n_{i}^{(\check{\alpha})})^{j} (s-s_0)^{j}.$$
The leading term  around $s=s_0$ of
$$\prod_{\alpha \in N_{0}(\chi_{s_{0}})}
\zeta(l_{\alpha}^{+}(\chi_{s}))$$ is the product of the leading term of every $\zeta(l_{\alpha}^{+}(\chi_{s}))$ around $s=s_0$. Therefore it equals to 
$$\prod_{\alpha \in N_{0}(\chi_{s_0})
	}\frac{1}{n_{i}^{(\check{\alpha})}
	}
	\times \left(\frac{R}{b_{ii}}\right)^{|N_{0}(\chi_{s_0})|} \times 
	(s-s_0)^{|N_{0}(\chi_{s_0})|}
	$$
Every $\alpha \in \Delta_{\para{P}}$ satisfies  
$\inner{\chi_{s},\check{\alpha}}=1$
Therefore by a similar argument 
$$\prod_{\tiny{
			\begin{aligned}
			\alpha \in N_{1}(\chi_{s_0}) \\
			\alpha \not \in \Delta_{\para{P}}\\
			\end{aligned}}}l_{\alpha}^{-}(\chi_s)=
				 \times 
b_{ii}^{|N_{1}(\chi_{s_0})|}
(s-s_0)^{|N_{1}(\chi_{s_0})|}
\times 
	\prod_{\tiny{
				\begin{aligned}
				\alpha \in N_{1}(\chi_{s_0}) \\
				\alpha \not \in \Delta_{\para{P}}\\
				\end{aligned}}				
				}
				n_{i}^{(\check{\alpha})}
 .$$
Hence, the leading term of $H(s)$ around $s=s_0$ is 
$$\epsilon_{s_0} \times R^{|N_{0}(\chi_{s_0})|}	\times (s-s_0)^{ |N_{1}(\chi_{s_0})| - |N_{0}(\chi_{s_0})|-(n-1)}$$
\end{enumerate}
\end{proof}
\end{lemm}
Let us recall Recall Proposition (\ref{ReducetoParabolic}) 
\begin{prop*}
Let $\para{P}=\para{P}_r$ be maximal parabolic of $G$.
	Let $\chi_{s}= \delta_{\para{P}}^{s-\frac{1}{2}}\otimes 
	\delta_{\para{B}}^{\frac{1}{2}}$  Then the  iterated  residue of $E_{\para{B}}(\chi,f^{0},g)$ along 
	$\mathcal{F}_{\hat{r}}=\mathcal{F}^{-}_{\alpha_1}, \dots, \mathcal{F}^{-}_{\alpha_{r-1}},\mathcal{F}_{\alpha_{r+1}}^{-},\dots ,\mathcal{F}^{-}_{\alpha_{n}}$
	is equal to $Res_{\mathcal{F}_{\hat{r}}} C_{\weylelement{_{\para{P}}}}(\chi) \times E_{\para{P}}(f^{0},s,g)
	$ where $\weylelement{_{\para{P}}}$ is the longest element in $\weyl{\para{P}}$. Moreover 
	$Res_{\mathcal{F}_{\hat{r}}} C_{\weylelement{\para{P}}}(\chi_s) \neq 0$ and is a constant function.
\end{prop*}


\begin{remk}\label{Lemma}
With the notations as above, $E_{\para{B}}^{\#}(\chi_s,g)$ can be written as 
 $$E_{\para{B}}^{\#}(\chi_s,g) = A_{\weylelement{\para{P}}} \times
 G(\chi_s)   \times \prod_{\alpha \in \Delta_{\para{P}}} \zeta(l_{\alpha}^{+}(\chi_s))l_{\alpha}^{+}(\chi_s) \times E_{\para{P}}(f^{0},s,g)
 $$
 where 
 $G(\chi_s)= \prod_{\alpha \in \Phi^{+} \setminus \Delta_{\para{P}}} \zeta(l_{\alpha}^{+}(\chi_s))
 l_{\alpha}^{+}(\chi_s)
 l_{\alpha}^{-}(\chi_s)$
 and $A_{\weylelement{\para{P}}}=Res_{\mathcal{F}_{\hat{i}}} C_{\weylelement{\para{P}}}(\chi_s)$.
\end{remk}
\iffalse
While $A_{\weylelement{\para{P}}}$ and 
$\prod_{\alpha \in \Delta_{\para{P}}} \zeta(l_{\alpha}^{+}(\chi_s))l_{\alpha}^{+}(\chi_s)$ are holomorphic and non zeros for all $s \in \mathbb{C}$,
 $G(s)$ admits a zero of order $|N_{1}(\chi_{s_0})| - |N_{0}(\chi_{s_0})|-(n-1)$ at $s=s_0$. Therefore, since $E_{\para{B}}^{\#}(\chi,g)$ is entire for every $\chi$
 in particular for $\chi = \chi_s$ 
  we get an upper bound for the pole order of $E_{\para{P}}(f^{0},g,s)$ at $s=s_0$
 this upper bound $d_{\para{P}}(\chi_{s_0})$ is equal to 
 $|N_{0}(\chi_{s_0})|-(n-1)$
 Now let us plug in all what we done until now to get the following Lemma.
 \fi
\begin{lemm}\label{LemmaT10}
Let $\para{P}=\para{P}_i$ be a maximal parabolic subgroup of $G$. 
Let $\chi_{s_0}=\delta_{\para{P}}^{s_0- \frac{1}{2}} \otimes \delta_{\para{B}}^{\frac{1}{2}}$.
With the same notations as above it holds that: 
%\begin{enumerate}
%\item
%The Eisenstein series $E_{\para{P}}(f^{0},s,g)$ admits a pole %of order at most $$d_{\para{P}}(\chi_{s_0}) =
%|N_{1}(\chi_{s_0})|-|N_{0}(\chi_{s_0})|- (n-1)
%$$
%at $s=s_0$.
%\item
\begin{align*}
E_{\para{B}}^{\#}(\chi_{s_0},g)=&(-1)^{|\Phi^{+}|+|N_{1}(\chi_{s_0})| + | N_{-1}(\chi_{s_0})|} \times h_3(\chi_{s_0}) \times h_4(\chi_{s_0}) \\
&\times 
R^{ | N_{0}(\chi_{s_0})| + |N_{-1}(\chi_{s_0})|} \times \epsilon_{s_0}
  \\
& \times
\zeta(2)^{|N_1(\chi_{s_0})|} \times 
(2)^{|N_{1}(\chi_{s_0})| + |N_{-1}(\chi_{s_0})|}
A_{\weylelement{_{\para{P}}}}
\leadingterm{-d_{\para{P}(\chi_{s_0})}}^{\para{P}}(f^{0},s_0,g)
\end{align*}
%\end{enumerate}
\end{lemm}
\iffalse
\begin{lemm}[Lemma T6]\label{Lemma-T8}
Let $\chi$ be a character of $T$. Then
\begin{align*}
E_{\para{B}}^{\#}(\chi,g)=&(-1)^{|\Phi^{+}|+|N_{-1}(\chi)|}\times h_3(\chi) h_4(\chi) \\
\times & \prod_{\alpha \in N_{1}(\chi)}l_{\alpha}^{+}(\chi) \zeta(l_{\alpha}^{+}(\chi)) \\
\times & \prod_{\alpha \in N_{0}(\chi)}l_{\alpha}^{+}(\chi) \zeta(l_{\alpha}^{+}(\chi)) \\
\times & \prod_{\alpha \in N_{-1}(\chi)}l_{\alpha}^{-}(\chi) \zeta(l_{\alpha}^{+}(\chi)) \\
\times & E_{\para{B}}(f^{0},\chi,g)
\end{align*}
\end{lemm}
\begin{proof}
\begin{align*}
E_{\para{B}}^{\#}(\chi,g)=
&\prod_{\alpha \in \Phi^{+}}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)E_{\para{B}}(f^{0},\chi,g)\\
=&   \prod_{\alpha \in N_{0}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)
 \times  \prod_{\alpha \in N_{1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi) \\
 & \times   \prod_{\alpha \in N_{-1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)
 \times  \prod_{0<\alpha \not \in N_{\pm 1, 0}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi) \times E_{\para{B}}(f^{0},\chi,g)\\
=&
\prod_{\alpha \in N_{0}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)
 \times  \prod_{\alpha \in N_{1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)\\
& \times  \prod_{\alpha \in N_{-1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)
 \times  \prod_{0<\alpha \not \in N_{\pm 1, 0}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)\times (-1) l_{-\alpha}^{+}(\chi) \times E_{\para{B}}(f^{0},\chi,g)\\
=&(-1)^{|\Phi^{+}|-|N_{\pm 1}(\chi)|} \times h_4(\chi)h_3(\chi)
\prod_{\alpha \in N_{0}(\chi)}\zeta(l_{\alpha}^{+}(\chi))
 \times  \prod_{\alpha \in N_{1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)\\
& \times  \prod_{\alpha \in N_{-1}(\chi)}\zeta(l_{\alpha}^{+}(\chi))l_{\alpha}^{+}(\chi)l_{\alpha}^{-}(\chi)\times
E_{\para{B}}(f^{0},\chi,g)\\
\end{align*}
\end{proof}
\fi
\begin{thm} \label{main_thm}
Let $\para{P}_i,\para{P}_j$ be a maximal parabolic subgroup of $G$. 
\iffalse
Let $b_{ii},b_{jj}\in \mathbb{C}$ such that $\delta_{\para{P}_i}=b_{ii}\fundamental{i},\:
\delta_{\para{P}_j}=b_{jj}\fundamental{j}$.
\fi
 Let $s_0,t_0\in \mathbb{C}$ such that
 $ \weylelement{}\chi_{s_0}=\chi_{t_0}$
  for some  $\weylelement{}\in \weyl{G}$.  where 
$\chi_{s_0}= \delta_{\para{P}_i}^{s_0-\frac{1}{2}}\otimes \delta_{\para{B}}^{\frac{1}{2}}$ and  \\
$\chi_{t_0}= \delta_{\para{P}_j}^{t_0-\frac{1}{2}}\otimes \delta_{\para{B}}^{\frac{1}{2}}$. 
Assume that $h_4(\chi_{s_0}) \neq 0$.
Then there exists $A \in \mathbb{C}$ such that
$$\leadingterm{-d_{\para{P}_i}(\chi_{s_0})}^{\para{P}_i}(f^{0}_{\para{P}_i},s_0,g)=A \leadingterm{
-d_{\para{P}_j}(\chi_{t_0})
} 
 ^{\para{P}_j}(f^{0}_{\para{P}_j},t_0,g). 
 \quad \forall g \in G
 $$
 Moreover,
 $$A= \frac{\epsilon_{t_0}}{\epsilon_{s_0}}\times 
 \prod_{\tiny {\begin{aligned}
   		\alpha \in \Phi^{+} \\
   		\alpha \not \in B_{\pm 1,0}(\chi_{s_0})\\
   		\weylelement{}\alpha <0
   		\end{aligned}}}
   \frac{
   	\zeta (\left \langle \chi_{s_0} ,\check{\alpha} \right \rangle)
   }{\zeta(
   \left \langle \chi_{s_0} ,\check{\alpha} \right \rangle+1)
 }
  \times 
 \left(
 \frac{R}{\zeta(2)} \right)^{d}\times \frac{A_{\para{P}_j}}{A_{\para{P}_i}}
 $$
 where 
 \begin{align*}
A_{\weylelement{\para{P}_i}}&=
Res_{\mathcal
{F}_{\hat{i}}} C_{\weylelement{\para{P}_i}} (\chi_{s_0}) & A_{\weylelement{\para{P}_j}}&=
Res_{\mathcal
{F}_{\hat{j}}} C_{\weylelement{\para{P}_j}} (\chi_{t_0})\\
\iffalse
\epsilon_s&=\prod_{\tiny \begin{aligned}
\gamma  \in& N_{1}(\chi_s)\\
\check{\gamma}=&\sum_{k=1}^{n} n_{k}^{\check{\gamma}}\check{\alpha}_i
\end{aligned}}
b_{ii}n_{i}^{\check{\gamma}}
\times \prod_{\tiny \begin{aligned}
\gamma  \in& N_{0}(\chi_s)\\
\check{\gamma}=&\sum_{k=1}^{n} n_{k}^{\check{\gamma}}\check{\alpha}_i
\end{aligned}}
\frac{1}{b_{ii}n_i^{\check{\gamma}}} 
&
\epsilon_t&=\prod_{\tiny \begin{aligned}
\gamma  \in& N_{1}(\chi_s)\\
\check{\gamma}=&\sum_{k=1}^{n} n_{k}^{\check{\gamma}}\check{\alpha}_k
\end{aligned}}
b_{jj}n_{j}^{\check{\gamma}}
\times \prod_{\tiny \begin{aligned}
\gamma  \in& N_{0}(\chi_{s_0})\\
\check{\gamma}=&\sum_{k=1}^{n} n_{k}^{\check{\gamma}}\check{\alpha}_k
\end{aligned}}
\frac{1}{b_{jj}n_j^{\check{\gamma}}} \\
\fi
d=&|N_{-1}(\chi_{t_0})|-|N_{-1}(\chi_{s_0})|
 \end{align*}
\end{thm}
\begin{proof}
Using Lemma (\ref{LemmaT10}) we obtained  that:
\begin{align*}
E_{\para{B}}^{\#}(\chi_{s_0},g)=&(-1)^{|\Phi^{+}|+|N_{1}(\chi_{s_0})| + | N_{-1}(\chi_{s_0})|} \times h_3(\chi_{s_0}) \times h_4(\chi_{s_0}) \\
&\times 
R^{ | N_{0}(\chi_{s_0})| + |N_{-1}(\chi_{s_0})|} \times \epsilon_{s_0}
\\
& \times
\zeta(2)^{|N_1(\chi_{s_0})|} \times 
(2)^{|N_{1}(\chi_{s_0})| + |N_{-1}(\chi_{s_0})|}
A_{\weylelement{_{\para{P}_i}}}
\leadingterm{-d_{\para{P}_i(\chi_{s_0})}}^{\para{P}_i}(f^{0},s_0,g)
\end{align*}
By a similar argument we get :
\begin{align*}
E_{\para{B}}^{\#}(\chi_{t_0},g)=&(-1)^{|\Phi^{+}|+|N_{1}(\chi_{t_0})| + | N_{-1}(\chi_{t_0})|} \times h_3(\chi_{t_0}) \times h_4(\chi_{t_0}) \\
&\times 
R^{ | N_{0}(\chi_{t_0})| + |N_{-1}(\chi_{t_0})|} \times \epsilon_{t_0}
\\
& \times
\zeta(2)^{|N_1(\chi_{t_0})|} \times 
(2)^{|N_{1}(\chi_{t_0})| + |N_{-1}(\chi_{t_0})|}
A_{\weylelement{_{\para{P}_j}}}
\leadingterm{-d_{\para{P}_j(\chi_{t_0})}}^{\para{P}_i}(f^{0},t_0,g)
\end{align*}
Since $E_{\para{B}}^{\#}$ is $W$-- invariant, both term are equal. So, we get:
\begin{align*}
\leadingterm{-d_{\para{P}_i}(\chi_{s_0})}^{\para{P}_i}(f^{0},s_0,g)&=
(-1)^{|N_{\pm 1}(\chi_{t_0})| -|N_{\pm 1}(\chi_{s_0})|}
\times 
\frac{h_3(\chi_{t_0})}{h_3(\chi_{s_0})} \times \frac{h_4(\chi_{t_0})}{h_4(\chi_{s_0})} \times \frac{\epsilon_{t_0}}{\epsilon_{s_0}} \\
& \times R^{|N_{-1}(\chi_{t_0})|-|N_{-1}(\chi_{s_0})| +
 |N_{0}(\chi_{t_0})|-|N_{0}(\chi_{s_0})| }
 \\
 &\times 2^{|N_{\pm 1}(\chi_{t_0})| -|N_{\pm 1}(\chi_{s_0})|} \times \zeta(2)^{|N_{1}(\chi_{t_0})| -|N_{1}(\chi_{s_0})|}  \\
 & \times 
\frac{A_{\weylelement{\para{P}_j}}}{A_{\weylelement{\para{P}_i}}} \times \leadingterm{-d_{\para{P}_j}(\chi_{t_0})}^{\para{P}_j}(f^{0},t_0,g)
\end{align*}
 Using Lemma (\ref{Size_Lemma}) it holds that:
 \begin{align*}
 (-1)^{|N_{\pm1}(\chi_{s_0})| - N_{\pm1}(\chi_{t_0})|} &= 1 &
 2^{|N_{\pm1}(\chi_{s_0})| - N_{\pm1}(\chi_{t_0})|} &= 1 &
R^{|N_{0}(\chi_{s_0})| - |N_{0}(\chi_{t_0})|} &=1 \\
   \end{align*}
Hence it holds that:
\begin{align*}
\leadingterm{-d_{\para{P}_i}(\chi_{s_0})}^{\para{P}_i}(f^{0},s_0,g)&=
\frac{h_3(\chi_{t_0})}{h_3(\chi_{s_0})} \times \frac{h_4(\chi_{t_0})}{h_4(\chi_{s_0})} \times \frac{\epsilon_{t_0}}{\epsilon_{s_0}} \\
& \times R^{|N_{-1}(\chi_{t_0})|-|N_{-1}(\chi_{s_0})|}
\\
&\times \zeta(2)^{|N_{1}(\chi_{t_0})| -|N_{1}(\chi_{s_0})|}  \\
& \times 
\frac{A_{\weylelement{\para{P}_j}}}{A_{\weylelement{\para{P}_i}}} \times \leadingterm{-d_{\para{P}_j}(\chi_{t_0})}^{\para{P}_j}(f^{0},t_0,g)
\end{align*}
Using corollary (\ref{cor_1}) and Lemma(\ref{Lemma-T4} ) it holds that
\begin{align*}
\frac{h_3(\chi_{t_0})}{h_3(\chi_{s_0})}&=1
&
R^{|N_{-1}(\chi_{t_0})| - |N_{-1}(\chi_{s_0})|} \times 
\zeta(2)^{|N_{-1}(\chi_{t_0})| - |N_{-1}(\chi_{s_0})|} &=
\left(\frac{R}{\zeta(2)}\right)^{d}
\end{align*}
Hence,
we obtain
 \begin{align*}
 \leadingterm{-d_{\para{P}_i}(\chi_{s_0})}^{\para{P}_i}(f^{0},s_0,g)&=  \frac{\epsilon_{t_0}}{\epsilon_{s_0}} 
  \times \left(\frac{R}{\zeta(2)}\right)^d
 \times
 \iffalse
 \prod_{\tiny {\begin{aligned}
 \alpha \in \Phi^{+} \\
 \alpha \not \in B_{\pm 1,0}(\chi_{s_0})\\
 \weylelement{}\alpha <0
 \end{aligned}}}
 \frac{
 \zeta (\left \langle \chi_{s_0} ,\check{\alpha} \right \rangle)
 }{\zeta(
 \left \langle \chi_{s_0} ,\check{\alpha} \right \rangle+1)
 }
 \fi
  \frac{h_4(\chi_{t_0})}{h_4(\chi_{s_0})}
  \times
 \frac{A_{\weylelement{\para{P}_j}}}{A_{\weylelement{\para{P}_i}}}  \times 
  \leadingterm{-d_{\para{P}_j}(\chi_{t_0})}^{\para{P}_j}(f^{0},t_0,g)
 \end{align*}
 Using Lemma (\ref{Lemma-T5})
  \begin{align*}
  \leadingterm{-d_{\para{P}_i}(\chi_{s_0})}^{\para{P}_i}(f^{0},s_0,g)&=  \frac{\epsilon_{t_0}}{\epsilon_{s_0}} 
  \times \left(\frac{R}{\zeta(2)}\right)^d
  \times
  \prod_{\tiny {\begin{aligned}
  		\alpha \in \Phi^{+} \\
  		\alpha \not \in B_{\pm 1,0}(\chi_{s_0})\\
  		\weylelement{}\alpha <0
  		\end{aligned}}}
  \frac{
  	\zeta (\left \langle \chi_{s_0} ,\check{\alpha} \right \rangle)
  }{\zeta(
  \left \langle \chi_{s_0} ,\check{\alpha} \right \rangle+1)
}
\iffalse
\frac{h_4(\chi_{t_0})}{h_4(\chi_{s_0})}
\fi
\times
\frac{A_{\weylelement{\para{P}_j}}}{A_{\weylelement{\para{P}_i}}}  \times 
\leadingterm{-d_{\para{P}_j}(\chi_{t_0})}^{\para{P}_j}(f^{0},t_0,g)
\end{align*}
 Observe that 
 \begin{align*}
 d_{\para{P}_i}(\chi_{s_0})-d=&
 |N_{1}(\chi_{s_0})| -
 |N_{0}(\chi_{s_0})|-(n-1)
 - |N_{-1}(\chi_{t_0})| + |N_{-1}(\chi_{s_0})|\\
 =&
 |N_{1}(\chi_{s_0})| -
 |N_{0}(\chi_{s_0})|-(n-1)
 + |N_{1}(\chi_{t_0})| - |N_{1}(\chi_{s_0})| \\
 =& |N_{1}(\chi_{t_0})| -|N_{0}(\chi_{s_0})| -(n-1) =d_{\para{P}_j}(\chi_{t_0})
 \end{align*}
\end{proof}

